Factorization systems on (stable) derivators

We define triangulated factorization systems on triangulated categories, and prove that a suitable subclass thereof (the normal triangulated torsion theories) corresponds bijectively to $t$-structures on the same category. This result is then placed in the framework of derivators regarding a triangulated category as the base of a stable derivator. More generally, we define derivator factorization systems in the 2-category $\mathrm{PDer}$, describing them as algebras for a suitable strict 2-monad (this result is of independent interest), and prove that a similar characterization still holds true: for a stable derivator $\mathbb D$, a suitable class of derivator factorization systems (the normal derivator torsion theories) correspond bijectively with $t$-structures on the base $\mathbb{D}(\mathbb{1})$ of the derivator. These two result can be regarded as the triangulated- and derivator- analogues, respectively, of the theorem that says that `$t$-structures are normal torsion theories' in the setting of stable $\infty$-categories, showing how the result remains true whatever the chosen model for stable homotopy theory is.

==> kodi/tikzlibrarykodi.bapto.code.tex <==
%% tikzlibrarykodi.bapto.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% βάπτω • (báptō)
%   1. I dip, submerge
%   2. I dye, colour
%   3. I baptise

% Bapto is a node labeling mechanism.
% It allows for non-invasive relabeling.

% TODO: update circuitry diagram
% ,-- input             input hook
% `-> dispatcher ----.  forwards according to
% ,---[overwrite]----'    label overwriting configuration
% `-> (name|alias|×)    to either name key, alias key or discarding the input

%==[ input stage ]==============================================================

\pgfqkeys{/bapto/input}{
  .forward to=/bapto/controller,
}

%==[ dispatching stage ]========================================================

% TODO: write feature test to verify trigger is protected by controller
%   from undue forwards.
\pgfqkeys{/bapto/overwrite}{.is choice,
  false/.style={/bapto/controller/.code={\tikz@fig@name\ifx\tikz@fig@name\empty
                                         \pgfqkeys{/bapto}{trigger={##1}}\fi},
                /bapto/dispatcher/.code={\tikz@fig@name\ifx\tikz@fig@name\empty
                                         \pgfqkeys{/tikz}{name=##1}\fi}},
  alias/.style={/bapto/controller/.code={\pgfqkeys{/bapto}{trigger={##1}}},
                /bapto/dispatcher/.code={\pgfqkeys{/tikz}{alias=##1}}},
  true/.style= {/bapto/controller/.code={\pgfqkeys{/bapto}{trigger={##1}}},
                /bapto/dispatcher/.code={\pgfqkeys{/tikz}{name=##1}}},
  false, % default is no name overwriting and no aliasing
}



==> kodi/tikzlibrarykodi.code.tex <==
%% tikzlibrarykodi.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% koDi stands for kommutative Diagramme für *TEX*.

%==[ dependencies graph ]=======================================================

% NOTE: arrow notation means targets require sources.

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%                                %  TikZ/pgf standard libraries
%      calc ------------------.  %
%      matrix -------------.  |  %
%                          |  |  %
%~~~~~~~~~~~~~~~~~~~~~~~~~~|~~|~~%
%                          |  |  %  koDi volatile layer: TikZ bugfixes
%      kodi.diorthono      |  |  %
%                          |  |  %
%~~~~~~~~~~~~~~~~~~~~~~~~~~|~~|~~%
%                          |  |  %  koDi inner layer: baseline features
%      kodi.ektropi ----.  |  |  %
%      kodi.bapto ------|  |  |  %
%      kodi.katharizo --|  |  |  %
%  ,-- kodi.koinos --.  |  |  |  %
%  |                 |  |  |  |  %
%~~|~~~~~~~~~~~~~~~~~|~~|~~|~~|~~%
%  |                 |  |  |  |  %  koDi middle layer: custom parsers
%  |-- kodi.mitra <--+--|--'  |  %
%  |-- kodi.ozos <---|  |     |  %
%  |-- kodi.velos <--'  |     |  %
%  |                    |     |  %
%~~|~~~~~~~~~~~~~~~~~~~~|~~~~~|~~%
%  |                    |     |  %  koDi outer layer: user interface
%  `-> kodi.ramma <-----'     |  %
%      kodi.mandyas <---------'  %  TODO: does mandyas depend upon ramma?
%                                %
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%

% Given the graph above, these suffice to encompass koDi:

\usetikzlibrary[kodi.diorthono]
\usetikzlibrary[kodi.ramma]
\usetikzlibrary[kodi.mandyas]



==> kodi/tikzlibrarykodi.diorthono.code.tex <==
%% tikzlibrarykodi.diorthono.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% διορθώνω • (diorthóno)
%   1. I correct
%   2. I mend
%   3. I repair

% Diorthono is a collection of bugfixes.

% Save catcode of @ to restore it at EOF.
\edef\kDAct{\catcode`@=\the\catcode`@\relax}
\catcode`@=11\relax

% The following code patches \pgfpathcurvebetweentime.
% See http://tex.stackexchange.com/a/271024/82186 for reference.
% Original fix by Mark Wibrow.
\def\pgf@@pathcurvebetweentime#1#2#3#4#5#6{%
  \pgfmathparse{#1}%
  \let\pgf@time@s=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgf@time@t=\pgfmathresult%
  \ifdim\pgf@time@s pt>\pgf@time@t pt\relax%
    \pgfmathsetmacro\pgf@time@s{1-#1}%
    \pgfmathsetmacro\pgf@time@t{1-#2}%
    \pgf@@@pathcurvebetweentime{#6}{#5}{#4}{#3}%
  \else%
    \pgf@@@pathcurvebetweentime{#3}{#4}{#5}{#6}%
  \fi%
}
\def\pgf@@@pathcurvebetweentime#1#2#3#4{%
\begingroup%
  % Get the curve Q from curve P for time 0 to t
  \pgfextract@process\Pa{#1}%
  \pgfextract@process\Pb{#2}%
  \pgfextract@process\Pc{#3}%
  \pgfextract@process\Pd{#4}%
  % Qa = Pa
  \pgfextract@process\Qa{\Pa}%
  % Qb = Pa + t*(Pb-Pa).
  \pgfextract@process\Qb{%
    \pgfpointadd{\Pa}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Pa}{\Pb}}}%
  }%
  % Qc = Qb + t*((Pb + t*(Pc-Pb)) - Qb)
  \pgfextract@process\Qc{%
    \pgfpointadd{\Qb}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Qb}{\pgfpointadd{\Pb}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Pb}{\Pc}}}}}}%
  }%
  % Qd = (1-t)^3*Pa + 3*t(1-t)^2*Pb + 3*t^2(1-t)*Pc + t^3*Pd.
  \pgfextract@process\Qd{\pgfpointcurveattime{\pgf@time@t}{\Pa}{\Pb}{\Pc}{\Pd}}% 
  %
  % Now get the curve R from the reversed curve Q for time 0 to 1-s/t
  \pgfmathdivide@{\pgf@time@s}{\pgf@time@t}%
  \pgfmathadd@{-\pgfmathresult}{1.0}%
  \let\pgf@time@s=\pgfmathresult%
  % Rd = Qd
  \pgfextract@process\Rd{\Qd}%
  % Rc = Qd + s*(Qc-Qd).
  \pgfextract@process\Rc{%
    \pgfpointadd{\Qd}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Qd}{\Qc}}}%
  }%
  % Rb = Rc + s*((Qc + s*(Qb-Qc)) - Rc)
  \pgfextract@process\Rb{%
    \pgfpointadd{\Rc}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Rc}{\pgfpointadd{\Qc}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Qc}{\Qb}}}}}}%
  }%
  % Ra = (1-s)^3*Qd + 3*s(1-s)^2*Qc + 3*s^2(1-s)*Qb + s^3*Qa.
  \pgfextract@process\Ra{\pgfpointcurveattime{\pgf@time@s}{\Qd}{\Qc}{\Qb}{\Qa}}% 
  \ifpgf@ignoremoveto\else\pgfpathmoveto{\Ra}\fi%
  \pgfpathcurveto{\Rb}{\Rc}{\Rd}%
\endgroup%
}

% Restore catcode of @.
\kDAct



==> kodi/tikzlibrarykodi.ektropi.code.tex <==
%% tikzlibrarykodi.ektropi.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% εκτροπή • (ektropí)
%   1. diversion
%   2. deflection
%   3. aberration

% Ektropi is a mechanism to hijack the /tikz/.unknown handler.
% It allows the addition of maximum priority paths in the key finding algorithm.
% The diversions are globally scoped, cumulative and removable.

% Save catcode of @ to restore it at EOF.
\edef\kDAct{\catcode`@=\the\catcode`@\relax}
\catcode`@=11\relax

%==[ handler restoring procedure ]==============================================

% The default handler's code is backed up as a token list at load time.
% NOTE: this has implications on loading order!
% TODO: figure out whether it safe or not to just assume no other package
%   does this kind dangerous of stuff.
% TODO: just in case, wrap the backup procedure inside a callable key.

\newtoks\kDEktropiDefaultToksBackup

\expandafter\expandafter
\expandafter\kDEktropiDefaultToksBackup
\expandafter\expandafter
\expandafter{\csname pgfk@/tikz/.unknown/.@body\endcsname}

\def\kDEktropiRestore{
  % Restore handler body.
  \def\kDAct{\pgfkeyssetvalue{/tikz/.unknown/.@body}}
  \expandafter\kDAct\expandafter{\the\kDEktropiDefaultToksBackup}
  % Restore handler macro.
  % NOTE: #s are doubled since we're inside \kDAct helper.
  \def\kDAct{\long\def\kDAct####1\pgfeov}
  \expandafter\kDAct\expandafter{\the\kDEktropiDefaultToksBackup}
  \pgfkeyslet{/tikz/.unknown/.@cmd}\kDAct
}

% This key is the user interface. Self explanatory.
\pgfkeys{/ektropi/restore/.code={\kDEktropiRestore}}

%==[ handler hacking procedure ]================================================

% This key is the user interface. It wraps the /tikz/.unknown handler code
% with a conditional that executes it only if the unknown key retrieval
% fails inside the path passed to /ektropi/add.
\pgfkeys{/ektropi/add/.style={
  /tikz/.unknown/.add code=
    {
      \let\tikz@key\pgfkeyscurrentname
      \pgfkeys{#1/\tikz@key/.try={##1}}
      \ifpgfkeyssuccess\else
    }{
      \fi
    }
  }
}

% Restore catcode of @.
\kDAct



==> kodi/tikzlibrarykodi.katharizo.code.tex <==
%% tikzlibrarykodi.katharizo.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% καθαρίζω • (katharízo)
%   1. clean, wash
%   2. peel, descale
%   3. (slang) kill

% Katharizo is a detokenization/sanitation mechanism.
% It produces "safe" strings from tokens.

% ,-- input          input hook
% `-> expander ---.  performs expansion according to
% ,---[expand]----'    macro expansion configuration
% `-> expanded ---.  pre-sanitation hook
% ,-- sanitizer <-'  performs detokenization and sanitation according to
% `---[replace]---.    character replacement configuration
% ,-- sanitized <-'  pre-output hook
% `-> output         output hook

%==[ input stage ]==============================================================

\pgfqkeys{/katharizo/input}{
  .forward to=/katharizo/expander
}

%==[ expansion stage ]==========================================================

\pgfqkeys{/katharizo/expand}{.is choice,
  once/.style={/katharizo/expander/.style={/katharizo/expanded/.expand once={##1}}},
  full/.style={/katharizo/expander/.style={/katharizo/expanded/.expanded={##1}}},
  none/.style={/katharizo/expander/.style={/katharizo/expanded={##1}}},
  none % default is no expansion
}

\pgfqkeys{/katharizo/expanded}{
  .forward to=/katharizo/sanitizer
}

%==[ sanitation stage ]=========================================================

\pgfqkeys{/katharizo}{
  replace charcode/.code args={#1 with #2}{%
    % TODO: would a \string be of any use? or at least a stringification?
    \pgfkeys{/katharizo/replacements/characters/#1/.initial={#2}}%
  },
  remove charcode/.style={/katharizo/replace charcode={{#1} with {}}},
  remove charcodes/.style args={#1}{%
    /katharizo/remove charcodes loop={#1 \kD},
  },
  remove charcodes loop/.code args={#1 #2\kD}{%
    % \message{|||#1|#2|||}
    \ifx\relax#1\else\pgfkeys{/katharizo/remove charcode={#1}}\fi
    \ifx\relax#2\else\pgfkeys{/katharizo/remove charcodes loop={#2\kD}}\fi
  },
  replace character/.code args={#1 with #2}{%
    \edef\kDFoo{\number`#1}% TODO: can I inline this?
    % TODO: would a \string be of any use? or at least a stringification?
    \pgfkeys{/katharizo/replacements/characters/\kDFoo/.initial={#2}}%
  },
  remove character/.style={/katharizo/replace character={{#1} with {}}},
  remove characters/.code args={#1#2}{%
    \ifx\relax#1\else\pgfkeys{/katharizo/remove character={#1}}\fi
    \ifx\relax#2\else\pgfkeys{/katharizo/remove characters={#2}}\fi
  },
  remove characters={(),.:},
  remove charcode=92,% \ backslash
}


\pgfqkeys{/katharizo}{
  sanitizer/.code={
    % TODO: token replacement routine? Would that be useful?
    \kDKatharizoStringify#1\kD
    \expandafter\kDKatharizoSanitize\the\kDKatharizoStringified\kD
    \pgfkeysalso{/katharizo/sanitized/.expanded=\the\kDKatharizoSanitized}
    % \message{^^J:::\the\kDKatharizoSanitized:::^^J}
  }
}

\pgfqkeys{/katharizo/sanitized}{
  .forward to=/katharizo/output
}

%==[ output stage ]=============================================================

% NOTE: this must be defined/hooked before calling input
\pgfqkeys{/katharizo/output}{
}

\newtoks\kDKatharizoStringified

\def\kDKatharizoStringify#1\kD{
  \def\kDFoo{#1}
  \edef\kDFoo{\meaning\kDFoo}
  \def\kDAct##1:->##2\kD{##2}
  \edef\kDFoo{\expandafter\kDAct\kDFoo\kD}
  \kDKatharizoStringified\expandafter{\kDFoo}
}

\newtoks\kDKatharizoSanitized

\def\kDKatharizoSanitize#1\kD{
  \pgfkeysifdefined{/katharizo/replacements/characters/32}%
    {\edef\kDKatharizoSSpace{\pgfkeysvalueof{/katharizo/replacements/characters/32}}}%
    {\edef\kDKatharizoSSpace{\space}}%
  \def\kDKatharizoSAppendSpace
    {\edef\kDAct{\noexpand\kDKatharizoSanitized={\the\kDKatharizoSanitized\kDKatharizoSSpace}}\kDAct}
  \kDKatharizoSanitized={}
  \kDKatharizoSString#1 \kD}% NOTE: the whitespace is a mandatory string terminator

\def\kDKatharizoSString#1 #2\kD{%
  \ifx\relax#1\else                       % if string head word is not empty
    \kDKatharizoSWord#1\kD                % parse string head word
    \if#2\space\else                      % if string tail is not the space terminator
      \ifx\relax#2\else                   %   if string tail is not empty
        \kDKatharizoSAppendSpace\fi\fi\fi %     append space substitute to output
  \ifx\relax#2\else                       % if string tail is not empty
    \kDKatharizoSString#2\kD\fi}          %   recurse on string tail

\def\kDKatharizoSWord#1#2\kD{%
  \kDKatharizoSCharacter#1\kD   % parse word head character
  \ifx\relax#2\else             % if word tail is not empty
    \kDKatharizoSWord#2\kD\fi}  %   recurse on word tail

\def\kDKatharizoSCharacter#1\kD{%
  \pgfkeysifdefined{/katharizo/replacements/characters/\number`#1}%
    {\edef\kDFoo{\pgfkeysvalueof{/katharizo/replacements/characters/\number`#1}}}%
    {\edef\kDFoo{#1}}%
  \edef\kDAct{\noexpand\kDKatharizoSanitized={\the\kDKatharizoSanitized\kDFoo}}%
  \kDAct}



==> kodi/tikzlibrarykodi.koinos.code.tex <==
%% tikzlibrarykodi.koinos.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% κοινός • (koinós)
%   1. shared
%   2. common
%   3. public

% Koinos implements or aliases some commonplace macros.

% This macro is the blank space token.
\bgroup
\def\:{\global\let\kDBlankSpace= }\:
\egroup

% Save catcode of @ to restore it later.
\edef\kDAct{\catcode`@=\the\catcode`@\relax}
\catcode`@=11\relax

% The next two macros both implement token gobbling.

% This "hard" version gobbles any token, ignoring whitespace.
\let\kDGobbleHardTok\pgfutil@gobble

% This "soft" version gobbles only whitespace.
% NOTE: this is just the identity macro. Fun fact.
\def\kDGobbleSoftTok#1{#1}

% The next two macros both implement the following logical condition:
%   if next token is #1 then #2 else #3

% This "hard" version ignores whitespace.
\let\kDIfNextHardCh\pgfutil@ifnextchar

% This "soft" version does not ignore whitespace.
\long\def\kDIfNextSoftCh#1#2#3{%
\let\kDINCToken= #1% <- MEMO: this space is crucial
\def\kDINCTrue{#2}\def\kDINCFalse{#3}%
\futurelet\kDINCTok\kDINC%
}

\def\kDINC{\ifx\kDINCTok\kDINCToken\let\kDINCFalse\kDINCTrue\fi\kDINCFalse}

% Restore catcode of @.
\kDAct

% This macro appends token list #1 to token list #2.
\def\kDAppend#1#2{\edef\kDAct{\noexpand#2={\the#2\the#1}}\kDAct}

% This macro tokenizes the stream into \kDOptTok
% until a group preceeding a ';' character is found;
% then it puts the group into \kDGrpTok and gobbles the ';'.
\def\kDFetchOptAndGrpThen#1%
  {\kDOptTok={}\kDGrpTok={}\kDFetchTilGrpThen{#1}}
  
\newtoks\kDOptTok
\newtoks\kDGrpTok

\def\kDFetchGrpThen#1#2{%
  \def\kDExit{#1}%
  \def\kDLoop{\kDFetchTilGrpThen{#1}}%
  \kDTmpTok={{#2}}%
  \kDIfNextHardCh;
    {\kDGrpTok\the\kDTmpTok\expandafter\kDExit\kDGobbleHardTok}
    {\kDAppend\kDTmpTok\kDOptTok\kDLoop}}

\newtoks\kDTmpTok

\def\kDFetchTilGrpThen#1#2#{%
  \kDTmpTok={#2}%
  \kDAppend\kDTmpTok\kDOptTok
  \kDFetchGrpThen{#1}}

% This macro removes trailing whitespace from token list #1.
% TODO: it seems to be expanding macros; investigate.
\def\kDTrimTrailingSpace#1{
\kDDetectTrailingSpace#1
\ifkDDTSHasTrail
\def\kDRTS##1 \kD{#1={##1}}
\edef\kDRTSAct{\noexpand\kDRTS\the#1\noexpand\kD}
\kDRTSAct
\fi
}

\def\kDDetectTrailingSpace#1%
{
\kDDTSPrevSpacefalse
\edef\kDAct{\noexpand\kDDTSGob\the#1\noexpand\kD}
\kDAct
}

\newif\ifkDDTSHasTrail

\def\kDDTSGob%
{\kDIfNextSoftCh\kD
  {\ifkDDTSPrevSpace\kDDTSHasTrailtrue\else\kDDTSHasTrailfalse\fi\kDGobbleHardTok}
  {\kDIfNextSoftCh\kDBlankSpace
    {\kDDTSPrevSpacetrue\expandafter\kDDTSGob\kDGobbleSoftTok}
    {\kDDTSPrevSpacefalse\expandafter\kDDTSGob\kDGobbleHardTok}}}

\newif\ifkDDTSPrevSpace

% This macro removes leading whitespace from token list #1.
\def\kDTrimLeadingSpace#1{
\def\kDAct##1\kD{#1={##1}}
\expandafter\kDGobbleSpaceThen
\expandafter\kDAct\the#1\kD
}

\def\kDGobbleSpaceThen#1%
{\kDIfNextHardCh\bgroup
  {\kDGSGroupThen#1}
  {\kDGSOtherThen#1}}

\def\kDGSGroupThen#1#2{#1{#2}}

\def\kDGSOtherThen#1#2{#1#2}

%===============================================================================

% macros for dumping, debugging and testing
% TODO: not sure I want to depend on these being in the sourcecode instead of
%   some external package integrated with a TeX unit testing suite.
%   I'll work in that direction.

\newif\ifkDDumping
\kDDumpingfalse

\newwrite\kDDumpFile

\def\kDDumpOpen%
{\ifkDDumping\immediate\openout\kDDumpFile=\jobname.yml\fi}

\def\kDDump#1%
{\ifkDDumping\immediate\write\kDDumpFile{#1}\fi}

\def\kDDumpClose%
{\ifkDDumping\closeout\kDDumpFile\fi}



==> kodi/tikzlibrarykodi.mandyas.code.tex <==
%% tikzlibrarykodi.mandyas.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% μανδύας • (mandýas)
%   1. cloak
%   2. mantle
%   3. dolman

% Mandias defines the aesthetics aspect of the user level functionality,
% together with some baseline configuration.

% TODO: clean these up
\usetikzlibrary[calc]
% \usetikzlibrary[decorations.pathreplacing]
% \usetikzlibrary{decorations.pathmorphing}
% \usetikzlibrary[decorations.markings]
% \usetikzlibrary[arrows.meta]

\pgfqkeys{/kD}{
%==[ universal styles ]=========================================================
  every diagram/.append style={},
  every layout/.append style={square},
  every object/.append style={},
  every arrow/.append style={
    >=stealth,
  },
  every label/.append style={
    auto,
    inner sep=0.5ex,
    font=\everymath\expandafter{\the\everymath\scriptstyle}
  },
%==[ arrow styles ]=============================================================
  /kD/arrows/.cd,
    crossing over/clearance/.initial=0.5ex,
    crossing over/color/.initial=white,
    crossing over/.style={
      /tikz/preaction={
        -,
        draw=\pgfkeysvalueof{/kD/arrows/crossing over/color},
        line width=\pgfkeysvalueof{/kD/arrows/crossing over/clearance},
      },
    },
    shove/.style={
      /tikz/transform canvas={
        /tikz/shift={($(\tikztostart)!#1!-90:(\tikztotarget)-(\tikztostart)$)}
      }
    },
    slide/.style={
      /tikz/transform canvas={
        /tikz/shift={($(\tikztostart)!#1!0:(\tikztotarget)-(\tikztostart)$)}
      }
    },
%==[ label styles ]=============================================================
  /kD/labels/.cd,
    mid/.style={
      /tikz/fill=white,
      /tikz/shape=circle,
      /tikz/anchor=center,
      /tikz/inner sep=.25ex
    },
%=[ objects styles ]============================================================
  /kD/objects/.cd,
    % TODO: reflect on these styles
    % rectangular/.style 2 args={
    %   /tikz/node distance=#2 and #1
    % },
    % square/.style={
    %   /kD/objects/rectangular={#1}{#1}
    % },
    % golden/.style={
    %   /kD/objects/rectangular={#1}{0.618*#1}
    % },
    % % comb/.style={
    % %   /kD/objects/rectangular={#1}{sqrt(3/4)*#1},
    % % },
    % % comb/.default=4em,
    % square/.default=4em,
    % golden/.default=4em,
%=[ lattice styles ]============================================================
  /kD/layouts/.cd,
    rectangular/.style 2 args={
      /tikz/column sep={#1,between origins},
      /tikz/row sep={#2,between origins},
    },
    square/.style={
      /kD/layouts/rectangular={#1}{#1}
    },
    golden/.style={
      /kD/layouts/rectangular={#1}{0.618*#1}
    },
    comb/.code args={#1step #2 angle #3}{
      % TODO: write better option parser
      \if\relax#1\pgfkeys{/kD/layouts/horizontal comb=step #2 angle #3}
      \else\pgfkeys{/kD/layouts/#1comb=step #2 angle #3}\fi
    },
    horizontal comb/.style args={step #1 angle #2}{
      /kD/layouts/rectangular={#1}{tan(#2)*#1*0.5},
      /tikz/every odd row/.append style={/tikz/xshift=(#1)*0.5}
    },
    vertical comb/.style args={step #1 angle #2}{
      /kD/layouts/rectangular={tan(#2)*#1*0.5}{#1},
      /tikz/every odd column/.append style={/tikz/yshift=-1*(#1)*0.5}
    },
    comb/.default=step 4.5em angle 60,
    horizontal comb/.default=step 4.5em angle 60,
    vertical comb/.default=step 4.5em angle 60,
    square/.default=4.5em,
    golden/.default=4.5em,
%=[ diagram styles ]============================================================
  /kD/diagrams/.cd,
    grid/.style 2 args={
      /tikz/x={#1},
      /tikz/y={#2},
      /tikz/on grid
    },
    metric/.style 2 args={
      % {1 and 1}{1} is infty-norm, unit circle is unit square
      % {2}{0.5} is 1-norm, circle of radius 2 is rhombus circumscribing base hexagon
      /tikz/node distance={#1},
      % TODO: implement control to allow for explicit units on single factor specs
      /tikz/above left/.code={\tikz@lib@place@handle@{##1}{south east}{-1}{1}{north west}{#2}},
      /tikz/above right/.code={\tikz@lib@place@handle@{##1}{south west}{1}{1}{north east}{#2}},
      /tikz/below left/.code={\tikz@lib@place@handle@{##1}{north east}{-1}{-1}{south west}{#2}},
      /tikz/below right/.code={\tikz@lib@place@handle@{##1}{north west}{1}{-1}{south east}{#2}}
    },
    rectangular/.style 2 args={
      /kD/every layout/.append style={/kD/layouts/rectangular={#1}{#2}},
      % TODO: how much of the following is necessary in layouts?
      /kD/diagrams/grid={#1}{#2},
      /kD/diagrams/metric={1 and 1}{1}
    },
    square/.style={
      /kD/every layout/.append style={/kD/layouts/square={#1}},
      /kD/diagrams/grid={#1}{#1},
      /kD/diagrams/metric={1 and 1}{1}
    },
    golden/.style={
      /kD/every layout/.append style={/kD/layouts/golden={#1}},
      /kD/diagrams/grid={#1}{0.618*#1},
      /kD/diagrams/metric={1 and 1}{1}
    },
    comb/.code args={#1step #2 angle #3}{
      % TODO: write better option parser
      \if\relax#1\pgfkeys{/kD/diagrams/horizontal comb=step #2 angle #3}
      \else\pgfkeys{/kD/diagrams/#1comb=step #2 angle #3}\fi
    },
    horizontal comb/.style args={step #1 angle #2}{
      /kD/every layout/.append style={/kD/layouts/horizontal comb=step #1 angle #2},
      /kD/diagrams/grid={#1*0.5}{#1*tan(#2)*0.5},
      /kD/diagrams/metric={2}{0.5}
    },
    vertical comb/.style args={step #1 angle #2}{
      /kD/every layout/.append style={/kD/layouts/vertical comb=step #1 angle #2},
      /kD/diagrams/grid={#1*tan(#2)*0.5}{#1*0.5},
      /kD/diagrams/metric={2}{0.5}
    },
    comb/.default=step 4.5em angle 60,
    rectangular/.default={6em}{4em},
    square/.default=4.5em,
    golden/.default=4.5em,
}



==> kodi/tikzlibrarykodi.mitra.code.tex <==
%% tikzlibrarykodi.mitra.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% μήτρα • (mítra)
%   1. womb
%   2. matrix
%   3. mold

% Mitra is an alternative parsing mechanism for TiKz matrices of nodes.
% It couples with ozos to ensure the node contents  always pass through the TikZ key.

\usetikzlibrary{matrix}
\usetikzlibrary{kodi.koinos}

%==[ TikZ/pgf layer ]===========================================================

\pgfkeys{
  /mitra/every matrix/.style={
    /tikz/matrix,
    /tikz/cells={
      /tikz/anchor=base
    }
  },
  /mitra/every node/.style={},
  % NOTE: the alisa key *cannot* be put along with global node styles
  %   because order of execution.
  /mitra/matrix coordinates alias/.style={
    /tikz/alias=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn,
  }
}

%==[ main macro ]===============================================================

\def\kDMitra
  {\kDMitraFetchMatrixThen
  {\kDMitraParseMatrixTableThen
   \kDMitraOutput}}

% General purpose scratch register.
\newtoks\kDMitraTmpTok

%==[ fetching routine ]=========================================================

% I use the general one implemented by koinos.
\let\kDMitraFetchMatrixThen\kDFetchOptAndGrpThen

%==[ parsing routine: /table ]==================================================

\newtoks\kDMitraMatOutTok

\def\kDMitraParseMatrixTableThen#1{%
  \kDMitraMatOutTok={}%
  \expandafter\kDMitraParseTable\the\kDGrpTok\kD
  #1}

\def\kDMitraParseTable
  {\kDMitraParseAllRowsThen\relax}

\def\kDMitraParseAllRowsThen#1{%
  \def\kDExit{#1}%
  \kDIfNextHardCh\kD
    {\expandafter\kDExit\kDGobbleHardTok}%
    {\kDMitraParseOneRowThen{\kDMitraParseAllRowsThen{#1}}}}

%==[ parsing routine: /table/row ]==============================================

\def\kDMitraParseOneRowThen#1%
  {\kDMitraMarkRowEndBefore
  {\kDMitraParseAllColsThen
  {\kDMitraParseRowEndThen
  {#1}}}}

\begingroup\catcode`&=4 % ConTeXt hack
\gdef\kDMitraMarkRowEndBefore#1#2\\{#1#2&\kD\\}
\endgroup

\def\kDMitraParseAllColsThen#1{%
  \def\kDExit{#1}%
  \kDIfNextHardCh\kD
    {\expandafter\kDExit\kDGobbleHardTok}%
    {\kDMitraParseOneColThen{\kDMitraParseAllColsThen{#1}}}}

\def\kDMitraParseRowEndThen#1%
  {\kDMitraFetchRowEndThen
  {\kDMitraPrintRowEndThen
  {#1}}}

\def\kDMitraFetchRowEndThen#1\\{\kDMitraMaybeFetchRowOptionsThen{#1}}

\newtoks\kDMitraRowOptTok

\def\kDMitraPrintRowEndThen#1{%
  \edef\kDAct{\noexpand\kDMitraTmpTok={\noexpand\\\the\kDMitraRowOptTok}}%
  \kDAct
  \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
  #1}

\def\kDMitraMaybeFetchRowOptionsThen#1{%
  \kDMitraRowOptTok={}%
  \kDIfNextHardCh[%
    {\kDMitraFetchRowOptionsThen{#1}}%
    {#1}}

\def\kDMitraFetchRowOptionsThen#1[#2]{\kDMitraRowOptTok={[#2]}#1}

%==[ parsing routine: /table/row/column ]=======================================

\def\kDMitraParseOneColThen#1%
  {\kDMitraParseCellThen
  {\kDMitraParseColEndThen
  {#1}}}

\def\kDMitraParseColEndThen#1%
  {\kDMitraMaybeFetchColOptionsThen
  {\kDMitraMaybePrintColEndThen
  {#1}}}

\newtoks\kDMitraColOptTok

\def\kDMitraMaybeFetchColOptionsThen#1{%
  \kDMitraColOptTok={}%
  \kDIfNextHardCh[%
    {\kDMitraFetchColOptionsThen{#1}}%
    {#1}}

\def\kDMitraFetchColOptionsThen#1[#2]{\kDMitraColOptTok={[#2]}#1}

% TODO: make catcode change temporary with wrapping group and global defs
%   making sure auxiliary macros aren't botched (and don't botch anything).
\catcode`&=\active
\def\kDMitraMaybePrintColEndThen#1{%
  \kDIfNextHardCh\kD
    {#1}%
    {%
      \edef\kDAct{\noexpand\kDMitraTmpTok={\noexpand&\the\kDMitraColOptTok}}%
      \kDAct
      \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
      #1%
    }}
\catcode`&=4

%==[ parsing routine: /table/row/column/cell ]==================================

\def\kDMitraParseCellThen#1%
  {\kDMitraMaybeFetchCellOptionsThen
  {\kDMitraFetchCellContentThen
  {\kDMitraPrintCellThen
  {#1}}}}

\newtoks\kDMitraCelOptTok

\def\kDMitraMaybeFetchCellOptionsThen#1{%
  \kDMitraCelOptTok={}%
  \kDIfNextHardCh|%
    {\kDMitraFetchCellOptionsThen{#1}}
    {#1}}

\def\kDMitraFetchCellOptionsThen#1|#2|{\kDMitraCelOptTok={#2}#1}

\newtoks\kDMitraCelCntTok

\def\kDMitraFetchCellContentThen#1#2&{%
  \kDMitraCelCntTok={#2}%
  \kDTrimLeadingSpace\kDMitraCelCntTok
  \kDTrimTrailingSpace\kDMitraCelCntTok
  #1}

\def\kDMitraMaybeDoCellThen#1{%
  \kDIfNextHardCh\kD
    {#1}%
    {\kDMitraParseOneColThen{#1}}}

\def\kDMitraPrintCellThen#1{%
  \edef\kDAct{%
    \noexpand\kDMitraTmpTok={%
      \noexpand\node
        [/mitra/every node]%
        \the\kDMitraCelOptTok
        [node contents={\the\kDMitraCelCntTok},%
        /mitra/matrix coordinates alias];% NOTE: be careful about placement
      \kDMitraMaybeDumpCell}}%
  \kDAct
  \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
  #1}

%==[ dumping routine ]==========================================================

% TODO: revise the mechanism
\def\kDMitraMaybeDumpCell{\noexpand\pgfextra{%
  \noexpand\kDDump{'\noexpand\the\noexpand\pgfmatrixcurrentrow-\noexpand\the\noexpand\pgfmatrixcurrentcolumn':}%
  \noexpand\kDDump{\space\space options: '\the\kDMitraCelOptTok'}%
  \noexpand\kDDump{\space\space content: '\the\kDMitraCelCntTok'}}}

%==[ output routine ]===========================================================

\def\kDMitraOutput{%
  \edef\kDAct{%
    \noexpand\kDMitraTmpTok={%
      \noexpand\matrix
        [/mitra/every matrix]%
        \the\kDOptTok
        {\the\kDMitraMatOutTok};}}%
  \kDAct
  \the\kDMitraTmpTok}

%==[ notes ]====================================================================

% \newif\ifConTeXt
% Trick stolen from iftex. The second line is expanded inside the group so
% the global scope isn't polluted by \csname defining the token.
% \begingroup\expandafter\expandafter\expandafter\endgroup\expandafter
%   \ifx\csname starttext\endcsname\relax\ConTeXtfalse\else\ConTeXttrue\fi
% \ifConTeXt\catcode`|=12 \fi% TODO: why was the space necessary again?



==> kodi/tikzlibrarykodi.ozos.code.tex <==
%% tikzlibrarykodi.ozos.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% όζος • (ózos)
%   1. node
%   2. nodule
%   3. gnarl

% Ozos is an alternative parsing mechanism for TiKz nodes.
% It implements the following transformation
%   \kDOzos ... {CONTENTS};  --->  \node ... [node contents={CONTENTS}];
% to ensure the node contents always pass through the TikZ key.

\usetikzlibrary{kodi.koinos}

%==[ TikZ/pgf layer ]===========================================================

\pgfkeys{/ozos/every node/.style={}}

%==[ main macro ]===============================================================

\def\kDOzos%
  {\kDOzosFetchThen
  {\kDOzosMaybeDumpThen
   \kDOzosOutput}}

%==[ fetching routine ]=========================================================

% I use the general one implemented by koinos.
\let\kDOzosFetchThen\kDFetchOptAndGrpThen

%==[ parsing routine ]==========================================================

% Trivially solved by fetching.

%==[ dumping routine ]==========================================================

% TODO: revise the mechanism
\def\kDOzosMaybeDumpThen#1{%
  \kDDump{options: '\the\kDOptTok'}%
  \kDDump{content: '\the\kDGrpTok'}%
  #1}

%==[ output routine ]===========================================================

\def\kDOzosOutput{
  \edef\kDAct{
    \noexpand\node
      [/ozos/every node]
      \the\kDOptTok
      [/tikz/node contents={\the\kDGrpTok}];
  }
  \kDAct
}



==> kodi/tikzlibrarykodi.ramma.code.tex <==
%% tikzlibrarykodi.ramma.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% ράμμα • (rámma)
%   1. suture
%   2. catgut
%   3. stitch

% Ramma ties together the lower level libraries to define
% the user level functionality. NOTE: strictly no aesthetics, see mandyas.

\usetikzlibrary[kodi.bapto]
\usetikzlibrary[kodi.ektropi]
\usetikzlibrary[kodi.katharizo]
\usetikzlibrary[kodi.koinos]
\usetikzlibrary[kodi.ozos]
\usetikzlibrary[kodi.mitra]
\usetikzlibrary[kodi.velos]

% And here is the core idea of koDi itself:

\pgfqkeys{/tikz}{% TODO: is this the best scope to put the key into?
  self naming/.style={
    /tikz/node contents/.forward to=/bapto/input,
    /bapto/trigger/.forward to=/katharizo/input,
    /katharizo/output/.forward to=/bapto/dispatcher
  }
}

% Some mischief with handlers and baseline math/labeling functionality.

\pgfqkeys{/kD}{
  .search also=/bapto,
  .search also=/katharizo,
  every thing/.style={
    /ektropi/restore,
    /ektropi/add=/kD,
    /ektropi/add=/bapto,
    /ektropi/add=/katharizo,
  },
  every diagram/.style={% NOTE: restore hopefully unnecessary
    /kD/every thing,
    /ektropi/add=/kD/diagrams,
  },
  every layout/.style={% NOTE: restore unnecessary
    /kD/every thing,
    /ektropi/add=/kD/layouts,
    nodes={/kD/every object}
  },
  every object/.style={% NOTE: needed when inside matrices
    /kD/every thing,
    /ektropi/add=/kD/objects,
    execute at begin node=$,%
    execute at end node=$,%
    self naming,
  },
  every arrow/.style={% NOTE: restore unnecessary
    /kD/every thing,
    /ektropi/add=/kD/arrows
  },
  every label/.style={% NOTE: restore needed because inside edge
    /kD/every thing,
    /ektropi/add=/kD/labels,
    execute at begin node=$,%
    execute at end node=$,%
    self naming
  }
}

% The user level keys are bound to the underlying parsers.

\pgfkeys{
  /mitra/every matrix/.append style=/kD/every layout,
  /ozos/every node/.append style=/kD/every object,
  /velos/every path/.append style={
    /tikz/every edge/.append style=/kD/every arrow,
    /tikz/every edge quotes/.append style=/kD/every label
  }
}

% I merge the macro syntax for objects and matrices. Convenient!

\newif\ifkDRammaObjIsMatrix

\def\kDRammaObjDecideWhetherIsMatrixThen#1{%
  \def\kDRammaObjDWIM{\kDRammaObjDWIMSightThen{\kDRammaObjDWIMGobThen{#1}}}%
  \expandafter\kDRammaObjDWIM\the\kDGrpTok\\\kD}

\def\kDRammaObjDWIMSightThen#1#2\\%
  {\kDIfNextHardCh\kD
    {\kDRammaObjIsMatrixfalse#1}%
    {\kDRammaObjIsMatrixtrue#1}}

\def\kDRammaObjDWIMGobThen#1#2\kD{#1}

\def\kDRammaObjOutput
  {\ifkDRammaObjIsMatrix
    \kDMitraParseMatrixTableThen\kDMitraOutput\else
    \kDOzosOutput\fi}

\def\kDRammaObj
  {\kDFetchOptAndGrpThen
  {\kDRammaObjDecideWhetherIsMatrixThen
   \kDRammaObjOutput}}

% Just an identity.
\let\kDRammaMor\kDVelos

% I envelope the koDi main macros in a simple key for maximal flexibility.

\tikzset{
  kodi/.code={%
    \catcode`\|=12% ConTeXt hack TODO: is it sufficient? investigate
    \let\obj\kDRammaObj
    \let\mor\kDRammaMor
  },
  kodi/.append style={/kD/every diagram}
}

% TODO: not convinced by the structure of what follows

%==[ main macro ]===============================================================

\def\kDRamma
  {\kDRammaMaybeFetchOptionsThen
   \kDRammaOutput}

%==[ fetching routine ]=========================================================

\newtoks\kDRammaOptTok
\newtoks\kDRammaTmpTok

\def\kDRammaMaybeFetchOptionsThen#1{%
  \kDRammaOptTok={}%
  \kDIfNextHardCh[%
    {\kDRammaFetchOptionsThen{#1}}%
    {#1}}

\def\kDRammaFetchOptionsThen#1[#2]{\kDRammaOptTok={#2}#1}

%==[ output routine ]===========================================================

\def\kDRammaOutput{%
  \edef\kDAct{%
    \noexpand\kDRammaTmpTok={%
      \noexpand\tikzpicture[kodi, \the\kDRammaOptTok]}}%
  \kDAct
  \the\kDRammaTmpTok}

\let\kDRammaOpen\kDRamma
\let\kDRammaShut\endtikzpicture



==> kodi/tikzlibrarykodi.velos.code.tex <==
%% tikzlibrarykodi.velos.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% βέλος • (vélos)
%   1. arrow
%   2. dart
%   3. shaft

% Velos is a parsing mechanism for arrow chains.

\usetikzlibrary{kodi.koinos}

%==[ handlers ]=================================================================

\pgfkeys{
  /velos/install quote handler/.style={
    /handlers/first char syntax=true,
    % TODO: verify if I can actually work w/quotes instead of against it
    /handlers/first char syntax/the character "/.initial=\kDVelosQuoteHandler
    % node quotes mean={node contents={#1}},
    % edge quotes mean={node contents={#1}}
  }
}

\def\kDVelosQuoteHandler#1%
  {\pgfkeysalso{/tikz/node contents/.expand once={\kDVelosUnquote#1}}}

\def\kDVelosUnquote"#1"{#1}

%==[ global options ]===========================================================

\newtoks\kDVelosTemp

\newtoks\kDVelosGlobalLabelOptions
\newtoks\kDVelosGlobalEdgeOptions

\newif\ifkDVelosGOAfterColon

\def\kDVelosFetchGlobalOptionsThen#1{%
  \kDVelosGOAfterColonfalse
  \kDVelosGlobalLabelOptions={}%
  \kDVelosGlobalEdgeOptions={}%
  \kDVelosGOMaybeFetchThen{\kDVelosGOThinkThen{#1}}}

\def\kDVelosGOMaybeFetchThen#1{%
  \kDVelosTemp={}%
  \kDIfNextHardCh[%
    {\kDVelosGOFetchThen{#1}}%
    {#1}}

\def\kDVelosGOFetchThen#1[#2]{%
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosGOThinkThen#1{%
  \def\kDVelosGOLoop{\kDVelosGOThinkThen{#1}}%
  \def\kDVelosGOBreak{#1}%
  \kDIfNextHardCh:%
    {%
      \kDVelosGOAfterColontrue
      \kDVelosGlobalLabelOptions\expandafter{\the\kDVelosTemp}%
      \expandafter\kDVelosGOMaybeFetchThen\expandafter\kDVelosGOLoop\kDGobbleHardTok
    }{%
      \ifkDVelosGOAfterColon
        \kDVelosGlobalEdgeOptions\expandafter{\the\kDVelosTemp}\else
        \kDVelosGlobalLabelOptions\expandafter{\the\kDVelosTemp}\fi
      \kDVelosGOBreak
    }}

%==[ first edge ]===============================================================

\def\kDVelosDoFirstEdgeThen#1%
  {\kDVelosFetchFirstSourceThen
  {\kDVelosFetchFirstEdgeThen
  {\kDVelosDrawFetchedEdgeThen
  {#1}}}}

\newtoks\kDVelosSource
\newtoks\kDVelosCurFstSrc
\newtoks\kDVelosPrvFstSrc

\def\kDVelosFetchFirstSourceThen#1%
  {\kDIfNextHardCh(%
    {\kDVelosFFSBracketsThen{#1}}%
    {\kDVelosFFSTillOverThen{#1}}}

\def\kDVelosFFSBracketsThen#1(#2){%
  \kDVelosSource={#2}%
  \kDVelosCurFstSrc={#2}%
  #1}

\def\kDVelosFFSTillOverThen#1#2 {% <- mind the space!
  \kDVelosSource={#2}%
  \kDVelosCurFstSrc={#2}%
  #1}

\def\kDVelosFetchFirstEdgeThen#1%
  {\kDVelosFetchEdgeThen
  {\kDVelosFetchTargetThen
  {#1}}}

%==[ chained edges ]============================================================

\newtoks\kDVelosEdge

\def\kDVelosFetchEdgeThen#1{%
  \kDVelosEdge={}%
  \kDVelosFEThen{\kDVelosFEThinkThen{#1}}}

\def\kDVelosFEThen#1%
  {\kDIfNextHardCh[%
    {\kDVelosFEKeysListThen{#1}}%
    {\kDIfNextHardCh"%
      {\kDVelosFEEnquotedThen{#1}}%
      {\kDVelosFETillOverThen{#1}}}}

\newif\ifkDVelosTempIsKeysList

\def\kDVelosFEEnquotedThen#1"#2"{%
  \kDVelosTempIsKeysListfalse
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosFEKeysListThen#1[#2]{%
  \kDVelosTempIsKeysListtrue
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosFETillOverThen#1{%
  \kDVelosTempIsKeysListfalse
  \kDVelosTemp={}%
  \kDVelosFETOThen{#1}}

\def\kDVelosFETOThen#1%
  {\kDIfNextSoftCh\kDBlankSpace
    {#1}%
    {\kDIfNextHardCh:%
      {#1}
      {\kDVelosFEAppendThen{\kDVelosFETOThen{#1}}}}}

\def\kDVelosFEAppendThen#1#2{%
  \kDVelosTemp=\expandafter{\the\kDVelosTemp#2}% TODO: wasn't the \ea redundant?
  #1}

\def\kDVelosFEEdgePrepend#1{%
  \edef\Act{\noexpand\kDVelosEdge={#1,\the\kDVelosEdge}}%
  \Act}

\def\kDVelosFEEdgePrependNode#1%
  {\kDVelosFEEdgePrepend{edge node={node[every edge quotes][/velos/install quote handler,#1]}}}
% TODO: install quote handler is maximally local to avoid conflict with quotes library;
%   is this the best handling of the situation?

\def\kDVelosFEThinkThen#1{%
  \def\kDVelosFELoop{\kDVelosFEThinkThen{#1}}%
  \def\kDVelosFEBreak{#1}%
  \kDIfNextHardCh[%
    {%
      \kDVelosFEEdgePrependNode{\the\kDVelosTemp}%
      \kDVelosFEThen\kDVelosFELoop
    }{%
      \kDIfNextHardCh:%
        {%
          \ifkDVelosTempIsKeysList
            \kDVelosFEEdgePrependNode{\the\kDVelosTemp}\else
            \kDVelosFEEdgePrependNode{"\the\kDVelosTemp"}\fi
          \expandafter\kDVelosFEThen\expandafter\kDVelosFELoop\kDGobbleHardTok
        }{%
          \kDVelosFEEdgePrepend{\the\kDVelosTemp}%
          \kDVelosFEBreak
        }%
    }}

%==[ target ]===================================================================

\newtoks\kDVelosTarget
\newtoks\kDVelosCurLstTar
\newtoks\kDVelosPrvLstTar

\def\kDVelosFetchTargetThen#1%
  {\kDIfNextHardCh(%
    {\kDVelosFTBracketsThen{#1}}%
    {\kDVelosFTTillOverThen{#1}}}

\def\kDVelosFTBracketsThen#1(#2){%
  \kDVelosTarget={#2}%
  \kDVelosCurLstTar={#2}%
  #1}

\def\kDVelosFTTillOverThen#1{%
  \kDVelosTarget={}%
  \kDVelosFTTOThen{#1}}

\def\kDVelosFTTOThen#1{%
  \def\kDVelosFTTOLoop%
    {\kDVelosFTTOThen{#1}}%
  \def\kDVelosFTTOExit{%
    \kDVelosCurLstTar\expandafter{\the\kDVelosTarget}%
    #1}%
  \kDIfNextSoftCh\kDBlankSpace
    {\kDVelosFTTOExit}%
    {\kDIfNextHardCh;%
      {\kDVelosFTTOExit}%
      {\kDVelosFTAppendThen\kDVelosFTTOLoop}}}

\def\kDVelosFTAppendThen#1#2{%
  \kDVelosTarget=\expandafter{\the\kDVelosTarget#2}%
  #1}

%==[ rendering/dereferencing ]==================================================

\def\kDVelosAlias{*}
\def\kDVelosSaila{+}

\newtoks\kDVelosDerefSrc
\newtoks\kDVelosDerefTar

\def\kDVelosDrawFetchedEdgeThen#1{
  \edef\cS{\the\kDVelosSource}%
  \kDVelosDerefSrc\expandafter{\the\kDVelosSource}%
  \ifx\cS\kDVelosAlias\kDVelosDerefSrc\expandafter{\the\kDVelosPrvFstSrc}\fi
  \ifx\cS\kDVelosSaila\kDVelosDerefSrc\expandafter{\the\kDVelosPrvLstTar}\fi
  \edef\cT{\the\kDVelosTarget}%
  \kDVelosDerefTar\expandafter{\the\kDVelosTarget}%
  \ifx\cT\kDVelosAlias\kDVelosDerefTar\expandafter{\the\kDVelosPrvLstTar}\fi
  \ifx\cT\kDVelosSaila\kDVelosDerefTar\expandafter{\the\kDVelosPrvFstSrc}\fi
  \edef\Act{%
    \noexpand\path
      [/velos/every path]%
      [%
        /tikz/every edge/.append style=%
          {\the\kDVelosGlobalEdgeOptions},%
        /tikz/every edge quotes/.append style=%
          {auto,\the\kDVelosGlobalLabelOptions},%
      ]%
      (\the\kDVelosDerefSrc)%
      edge[\the\kDVelosEdge]%
      (\the\kDVelosDerefTar);}%
  \Act%
  #1}

\pgfkeys{
  /velos/every path/.style={
    /velos/install quote handler
  }
}

%==[ high level ]===============================================================

\def\kDVelos%
  {\kDVelosFetchGlobalOptionsThen
  {\kDVelosDoFirstEdgeThen
   \kDVelosMaybeChainEdge}}

\def\kDVelosMaybeChainEdge{%
  \kDIfNextHardCh;%
    {%
    \edef\cS{\the\kDVelosCurFstSrc}%
    \ifx\cS\kDVelosAlias
      \kDVelosCurFstSrc\expandafter{\the\kDVelosPrvFstSrc}%
    \else\ifx\cS\kDVelosSaila
      \kDVelosCurFstSrc\expandafter{\the\kDVelosPrvLstTar}%
    \fi\fi
    \edef\cT{\the\kDVelosCurLstTar}%
    \ifx\cT\kDVelosAlias
      \kDVelosCurLstTar\expandafter{\the\kDVelosPrvLstTar}%
    \else\ifx\cT\kDVelosSaila
      \kDVelosCurLstTar\expandafter{\the\kDVelosPrvFstSrc}%
    \fi\fi
    \kDVelosPrvFstSrc\expandafter{\the\kDVelosCurFstSrc}%
    \kDVelosPrvLstTar\expandafter{\the\kDVelosCurLstTar}%
    }{%
      \kDVelosSource\expandafter{\the\kDVelosTarget}
      \kDVelosFetchEdgeThen
        {\kDVelosFetchTargetThen
        {\kDVelosDrawFetchedEdgeThen
         \kDVelosMaybeChainEdge}}%
    }}



==> tikzlibrarykodi.bapto.code.tex <==
%% tikzlibrarykodi.bapto.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% βάπτω • (báptō)
%   1. I dip, submerge
%   2. I dye, colour
%   3. I baptise

% Bapto is a node labeling mechanism.
% It allows for non-invasive relabeling.

% TODO: update circuitry diagram
% ,-- input             input hook
% `-> dispatcher ----.  forwards according to
% ,---[overwrite]----'    label overwriting configuration
% `-> (name|alias|×)    to either name key, alias key or discarding the input

%==[ input stage ]==============================================================

\pgfqkeys{/bapto/input}{
  .forward to=/bapto/controller,
}

%==[ dispatching stage ]========================================================

% TODO: write feature test to verify trigger is protected by controller
%   from undue forwards.
\pgfqkeys{/bapto/overwrite}{.is choice,
  false/.style={/bapto/controller/.code={\tikz@fig@name\ifx\tikz@fig@name\empty
                                         \pgfqkeys{/bapto}{trigger={##1}}\fi},
                /bapto/dispatcher/.code={\tikz@fig@name\ifx\tikz@fig@name\empty
                                         \pgfqkeys{/tikz}{name=##1}\fi}},
  alias/.style={/bapto/controller/.code={\pgfqkeys{/bapto}{trigger={##1}}},
                /bapto/dispatcher/.code={\pgfqkeys{/tikz}{alias=##1}}},
  true/.style= {/bapto/controller/.code={\pgfqkeys{/bapto}{trigger={##1}}},
                /bapto/dispatcher/.code={\pgfqkeys{/tikz}{name=##1}}},
  false, % default is no name overwriting and no aliasing
}



==> tikzlibrarykodi.code.tex <==
%% tikzlibrarykodi.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% koDi stands for kommutative Diagramme für *TEX*.

%==[ dependencies graph ]=======================================================

% NOTE: arrow notation means targets require sources.

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%                                %  TikZ/pgf standard libraries
%      calc ------------------.  %
%      matrix -------------.  |  %
%                          |  |  %
%~~~~~~~~~~~~~~~~~~~~~~~~~~|~~|~~%
%                          |  |  %  koDi volatile layer: TikZ bugfixes
%      kodi.diorthono      |  |  %
%                          |  |  %
%~~~~~~~~~~~~~~~~~~~~~~~~~~|~~|~~%
%                          |  |  %  koDi inner layer: baseline features
%      kodi.ektropi ----.  |  |  %
%      kodi.bapto ------|  |  |  %
%      kodi.katharizo --|  |  |  %
%  ,-- kodi.koinos --.  |  |  |  %
%  |                 |  |  |  |  %
%~~|~~~~~~~~~~~~~~~~~|~~|~~|~~|~~%
%  |                 |  |  |  |  %  koDi middle layer: custom parsers
%  |-- kodi.mitra <--+--|--'  |  %
%  |-- kodi.ozos <---|  |     |  %
%  |-- kodi.velos <--'  |     |  %
%  |                    |     |  %
%~~|~~~~~~~~~~~~~~~~~~~~|~~~~~|~~%
%  |                    |     |  %  koDi outer layer: user interface
%  `-> kodi.ramma <-----'     |  %
%      kodi.mandyas <---------'  %  TODO: does mandyas depend upon ramma?
%                                %
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%

% Given the graph above, these suffice to encompass koDi:

\usetikzlibrary[kodi.diorthono]
\usetikzlibrary[kodi.ramma]
\usetikzlibrary[kodi.mandyas]



==> tikzlibrarykodi.diorthono.code.tex <==
%% tikzlibrarykodi.diorthono.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% διορθώνω • (diorthóno)
%   1. I correct
%   2. I mend
%   3. I repair

% Diorthono is a collection of bugfixes.

% Save catcode of @ to restore it at EOF.
\edef\kDAct{\catcode`@=\the\catcode`@\relax}
\catcode`@=11\relax

% The following code patches \pgfpathcurvebetweentime.
% See http://tex.stackexchange.com/a/271024/82186 for reference.
% Original fix by Mark Wibrow.
\def\pgf@@pathcurvebetweentime#1#2#3#4#5#6{%
  \pgfmathparse{#1}%
  \let\pgf@time@s=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgf@time@t=\pgfmathresult%
  \ifdim\pgf@time@s pt>\pgf@time@t pt\relax%
    \pgfmathsetmacro\pgf@time@s{1-#1}%
    \pgfmathsetmacro\pgf@time@t{1-#2}%
    \pgf@@@pathcurvebetweentime{#6}{#5}{#4}{#3}%
  \else%
    \pgf@@@pathcurvebetweentime{#3}{#4}{#5}{#6}%
  \fi%
}
\def\pgf@@@pathcurvebetweentime#1#2#3#4{%
\begingroup%
  % Get the curve Q from curve P for time 0 to t
  \pgfextract@process\Pa{#1}%
  \pgfextract@process\Pb{#2}%
  \pgfextract@process\Pc{#3}%
  \pgfextract@process\Pd{#4}%
  % Qa = Pa
  \pgfextract@process\Qa{\Pa}%
  % Qb = Pa + t*(Pb-Pa).
  \pgfextract@process\Qb{%
    \pgfpointadd{\Pa}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Pa}{\Pb}}}%
  }%
  % Qc = Qb + t*((Pb + t*(Pc-Pb)) - Qb)
  \pgfextract@process\Qc{%
    \pgfpointadd{\Qb}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Qb}{\pgfpointadd{\Pb}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Pb}{\Pc}}}}}}%
  }%
  % Qd = (1-t)^3*Pa + 3*t(1-t)^2*Pb + 3*t^2(1-t)*Pc + t^3*Pd.
  \pgfextract@process\Qd{\pgfpointcurveattime{\pgf@time@t}{\Pa}{\Pb}{\Pc}{\Pd}}% 
  %
  % Now get the curve R from the reversed curve Q for time 0 to 1-s/t
  \pgfmathdivide@{\pgf@time@s}{\pgf@time@t}%
  \pgfmathadd@{-\pgfmathresult}{1.0}%
  \let\pgf@time@s=\pgfmathresult%
  % Rd = Qd
  \pgfextract@process\Rd{\Qd}%
  % Rc = Qd + s*(Qc-Qd).
  \pgfextract@process\Rc{%
    \pgfpointadd{\Qd}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Qd}{\Qc}}}%
  }%
  % Rb = Rc + s*((Qc + s*(Qb-Qc)) - Rc)
  \pgfextract@process\Rb{%
    \pgfpointadd{\Rc}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Rc}{\pgfpointadd{\Qc}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Qc}{\Qb}}}}}}%
  }%
  % Ra = (1-s)^3*Qd + 3*s(1-s)^2*Qc + 3*s^2(1-s)*Qb + s^3*Qa.
  \pgfextract@process\Ra{\pgfpointcurveattime{\pgf@time@s}{\Qd}{\Qc}{\Qb}{\Qa}}% 
  \ifpgf@ignoremoveto\else\pgfpathmoveto{\Ra}\fi%
  \pgfpathcurveto{\Rb}{\Rc}{\Rd}%
\endgroup%
}

% Restore catcode of @.
\kDAct



==> tikzlibrarykodi.ektropi.code.tex <==
%% tikzlibrarykodi.ektropi.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% εκτροπή • (ektropí)
%   1. diversion
%   2. deflection
%   3. aberration

% Ektropi is a mechanism to hijack the /tikz/.unknown handler.
% It allows the addition of maximum priority paths in the key finding algorithm.
% The diversions are globally scoped, cumulative and removable.

% Save catcode of @ to restore it at EOF.
\edef\kDAct{\catcode`@=\the\catcode`@\relax}
\catcode`@=11\relax

%==[ handler restoring procedure ]==============================================

% The default handler's code is backed up as a token list at load time.
% NOTE: this has implications on loading order!
% TODO: figure out whether it safe or not to just assume no other package
%   does this kind dangerous of stuff.
% TODO: just in case, wrap the backup procedure inside a callable key.

\newtoks\kDEktropiDefaultToksBackup

\expandafter\expandafter
\expandafter\kDEktropiDefaultToksBackup
\expandafter\expandafter
\expandafter{\csname pgfk@/tikz/.unknown/.@body\endcsname}

\def\kDEktropiRestore{
  % Restore handler body.
  \def\kDAct{\pgfkeyssetvalue{/tikz/.unknown/.@body}}
  \expandafter\kDAct\expandafter{\the\kDEktropiDefaultToksBackup}
  % Restore handler macro.
  % NOTE: #s are doubled since we're inside \kDAct helper.
  \def\kDAct{\long\def\kDAct####1\pgfeov}
  \expandafter\kDAct\expandafter{\the\kDEktropiDefaultToksBackup}
  \pgfkeyslet{/tikz/.unknown/.@cmd}\kDAct
}

% This key is the user interface. Self explanatory.
\pgfkeys{/ektropi/restore/.code={\kDEktropiRestore}}

%==[ handler hacking procedure ]================================================

% This key is the user interface. It wraps the /tikz/.unknown handler code
% with a conditional that executes it only if the unknown key retrieval
% fails inside the path passed to /ektropi/add.
\pgfkeys{/ektropi/add/.style={
  /tikz/.unknown/.add code=
    {
      \let\tikz@key\pgfkeyscurrentname
      \pgfkeys{#1/\tikz@key/.try={##1}}
      \ifpgfkeyssuccess\else
    }{
      \fi
    }
  }
}

% Restore catcode of @.
\kDAct



==> tikzlibrarykodi.katharizo.code.tex <==
%% tikzlibrarykodi.katharizo.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% καθαρίζω • (katharízo)
%   1. clean, wash
%   2. peel, descale
%   3. (slang) kill

% Katharizo is a detokenization/sanitation mechanism.
% It produces "safe" strings from tokens.

% ,-- input          input hook
% `-> expander ---.  performs expansion according to
% ,---[expand]----'    macro expansion configuration
% `-> expanded ---.  pre-sanitation hook
% ,-- sanitizer <-'  performs detokenization and sanitation according to
% `---[replace]---.    character replacement configuration
% ,-- sanitized <-'  pre-output hook
% `-> output         output hook

%==[ input stage ]==============================================================

\pgfqkeys{/katharizo/input}{
  .forward to=/katharizo/expander
}

%==[ expansion stage ]==========================================================

\pgfqkeys{/katharizo/expand}{.is choice,
  once/.style={/katharizo/expander/.style={/katharizo/expanded/.expand once={##1}}},
  full/.style={/katharizo/expander/.style={/katharizo/expanded/.expanded={##1}}},
  none/.style={/katharizo/expander/.style={/katharizo/expanded={##1}}},
  none % default is no expansion
}

\pgfqkeys{/katharizo/expanded}{
  .forward to=/katharizo/sanitizer
}

%==[ sanitation stage ]=========================================================

\pgfqkeys{/katharizo}{
  replace charcode/.code args={#1 with #2}{%
    % TODO: would a \string be of any use? or at least a stringification?
    \pgfkeys{/katharizo/replacements/characters/#1/.initial={#2}}%
  },
  remove charcode/.style={/katharizo/replace charcode={{#1} with {}}},
  remove charcodes/.style args={#1}{%
    /katharizo/remove charcodes loop={#1 \kD},
  },
  remove charcodes loop/.code args={#1 #2\kD}{%
    % \message{|||#1|#2|||}
    \ifx\relax#1\else\pgfkeys{/katharizo/remove charcode={#1}}\fi
    \ifx\relax#2\else\pgfkeys{/katharizo/remove charcodes loop={#2\kD}}\fi
  },
  replace character/.code args={#1 with #2}{%
    \edef\kDFoo{\number`#1}% TODO: can I inline this?
    % TODO: would a \string be of any use? or at least a stringification?
    \pgfkeys{/katharizo/replacements/characters/\kDFoo/.initial={#2}}%
  },
  remove character/.style={/katharizo/replace character={{#1} with {}}},
  remove characters/.code args={#1#2}{%
    \ifx\relax#1\else\pgfkeys{/katharizo/remove character={#1}}\fi
    \ifx\relax#2\else\pgfkeys{/katharizo/remove characters={#2}}\fi
  },
  remove characters={(),.:},
  remove charcode=92,% \ backslash
}


\pgfqkeys{/katharizo}{
  sanitizer/.code={
    % TODO: token replacement routine? Would that be useful?
    \kDKatharizoStringify#1\kD
    \expandafter\kDKatharizoSanitize\the\kDKatharizoStringified\kD
    \pgfkeysalso{/katharizo/sanitized/.expanded=\the\kDKatharizoSanitized}
    % \message{^^J:::\the\kDKatharizoSanitized:::^^J}
  }
}

\pgfqkeys{/katharizo/sanitized}{
  .forward to=/katharizo/output
}

%==[ output stage ]=============================================================

% NOTE: this must be defined/hooked before calling input
\pgfqkeys{/katharizo/output}{
}

\newtoks\kDKatharizoStringified

\def\kDKatharizoStringify#1\kD{
  \def\kDFoo{#1}
  \edef\kDFoo{\meaning\kDFoo}
  \def\kDAct##1:->##2\kD{##2}
  \edef\kDFoo{\expandafter\kDAct\kDFoo\kD}
  \kDKatharizoStringified\expandafter{\kDFoo}
}

\newtoks\kDKatharizoSanitized

\def\kDKatharizoSanitize#1\kD{
  \pgfkeysifdefined{/katharizo/replacements/characters/32}%
    {\edef\kDKatharizoSSpace{\pgfkeysvalueof{/katharizo/replacements/characters/32}}}%
    {\edef\kDKatharizoSSpace{\space}}%
  \def\kDKatharizoSAppendSpace
    {\edef\kDAct{\noexpand\kDKatharizoSanitized={\the\kDKatharizoSanitized\kDKatharizoSSpace}}\kDAct}
  \kDKatharizoSanitized={}
  \kDKatharizoSString#1 \kD}% NOTE: the whitespace is a mandatory string terminator

\def\kDKatharizoSString#1 #2\kD{%
  \ifx\relax#1\else                       % if string head word is not empty
    \kDKatharizoSWord#1\kD                % parse string head word
    \if#2\space\else                      % if string tail is not the space terminator
      \ifx\relax#2\else                   %   if string tail is not empty
        \kDKatharizoSAppendSpace\fi\fi\fi %     append space substitute to output
  \ifx\relax#2\else                       % if string tail is not empty
    \kDKatharizoSString#2\kD\fi}          %   recurse on string tail

\def\kDKatharizoSWord#1#2\kD{%
  \kDKatharizoSCharacter#1\kD   % parse word head character
  \ifx\relax#2\else             % if word tail is not empty
    \kDKatharizoSWord#2\kD\fi}  %   recurse on word tail

\def\kDKatharizoSCharacter#1\kD{%
  \pgfkeysifdefined{/katharizo/replacements/characters/\number`#1}%
    {\edef\kDFoo{\pgfkeysvalueof{/katharizo/replacements/characters/\number`#1}}}%
    {\edef\kDFoo{#1}}%
  \edef\kDAct{\noexpand\kDKatharizoSanitized={\the\kDKatharizoSanitized\kDFoo}}%
  \kDAct}



==> tikzlibrarykodi.koinos.code.tex <==
%% tikzlibrarykodi.koinos.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% κοινός • (koinós)
%   1. shared
%   2. common
%   3. public

% Koinos implements or aliases some commonplace macros.

% This macro is the blank space token.
\bgroup
\def\:{\global\let\kDBlankSpace= }\:
\egroup

% Save catcode of @ to restore it later.
\edef\kDAct{\catcode`@=\the\catcode`@\relax}
\catcode`@=11\relax

% The next two macros both implement token gobbling.

% This "hard" version gobbles any token, ignoring whitespace.
\let\kDGobbleHardTok\pgfutil@gobble

% This "soft" version gobbles only whitespace.
% NOTE: this is just the identity macro. Fun fact.
\def\kDGobbleSoftTok#1{#1}

% The next two macros both implement the following logical condition:
%   if next token is #1 then #2 else #3

% This "hard" version ignores whitespace.
\let\kDIfNextHardCh\pgfutil@ifnextchar

% This "soft" version does not ignore whitespace.
\long\def\kDIfNextSoftCh#1#2#3{%
\let\kDINCToken= #1% <- MEMO: this space is crucial
\def\kDINCTrue{#2}\def\kDINCFalse{#3}%
\futurelet\kDINCTok\kDINC%
}

\def\kDINC{\ifx\kDINCTok\kDINCToken\let\kDINCFalse\kDINCTrue\fi\kDINCFalse}

% Restore catcode of @.
\kDAct

% This macro appends token list #1 to token list #2.
\def\kDAppend#1#2{\edef\kDAct{\noexpand#2={\the#2\the#1}}\kDAct}

% This macro tokenizes the stream into \kDOptTok
% until a group preceeding a ';' character is found;
% then it puts the group into \kDGrpTok and gobbles the ';'.
\def\kDFetchOptAndGrpThen#1%
  {\kDOptTok={}\kDGrpTok={}\kDFetchTilGrpThen{#1}}
  
\newtoks\kDOptTok
\newtoks\kDGrpTok

\def\kDFetchGrpThen#1#2{%
  \def\kDExit{#1}%
  \def\kDLoop{\kDFetchTilGrpThen{#1}}%
  \kDTmpTok={{#2}}%
  \kDIfNextHardCh;
    {\kDGrpTok\the\kDTmpTok\expandafter\kDExit\kDGobbleHardTok}
    {\kDAppend\kDTmpTok\kDOptTok\kDLoop}}

\newtoks\kDTmpTok

\def\kDFetchTilGrpThen#1#2#{%
  \kDTmpTok={#2}%
  \kDAppend\kDTmpTok\kDOptTok
  \kDFetchGrpThen{#1}}

% This macro removes trailing whitespace from token list #1.
% TODO: it seems to be expanding macros; investigate.
\def\kDTrimTrailingSpace#1{
\kDDetectTrailingSpace#1
\ifkDDTSHasTrail
\def\kDRTS##1 \kD{#1={##1}}
\edef\kDRTSAct{\noexpand\kDRTS\the#1\noexpand\kD}
\kDRTSAct
\fi
}

\def\kDDetectTrailingSpace#1%
{
\kDDTSPrevSpacefalse
\edef\kDAct{\noexpand\kDDTSGob\the#1\noexpand\kD}
\kDAct
}

\newif\ifkDDTSHasTrail

\def\kDDTSGob%
{\kDIfNextSoftCh\kD
  {\ifkDDTSPrevSpace\kDDTSHasTrailtrue\else\kDDTSHasTrailfalse\fi\kDGobbleHardTok}
  {\kDIfNextSoftCh\kDBlankSpace
    {\kDDTSPrevSpacetrue\expandafter\kDDTSGob\kDGobbleSoftTok}
    {\kDDTSPrevSpacefalse\expandafter\kDDTSGob\kDGobbleHardTok}}}

\newif\ifkDDTSPrevSpace

% This macro removes leading whitespace from token list #1.
\def\kDTrimLeadingSpace#1{
\def\kDAct##1\kD{#1={##1}}
\expandafter\kDGobbleSpaceThen
\expandafter\kDAct\the#1\kD
}

\def\kDGobbleSpaceThen#1%
{\kDIfNextHardCh\bgroup
  {\kDGSGroupThen#1}
  {\kDGSOtherThen#1}}

\def\kDGSGroupThen#1#2{#1{#2}}

\def\kDGSOtherThen#1#2{#1#2}

%===============================================================================

% macros for dumping, debugging and testing
% TODO: not sure I want to depend on these being in the sourcecode instead of
%   some external package integrated with a TeX unit testing suite.
%   I'll work in that direction.

\newif\ifkDDumping
\kDDumpingfalse

\newwrite\kDDumpFile

\def\kDDumpOpen%
{\ifkDDumping\immediate\openout\kDDumpFile=\jobname.yml\fi}

\def\kDDump#1%
{\ifkDDumping\immediate\write\kDDumpFile{#1}\fi}

\def\kDDumpClose%
{\ifkDDumping\closeout\kDDumpFile\fi}



==> tikzlibrarykodi.mandyas.code.tex <==
%% tikzlibrarykodi.mandyas.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% μανδύας • (mandýas)
%   1. cloak
%   2. mantle
%   3. dolman

% Mandias defines the aesthetics aspect of the user level functionality,
% together with some baseline configuration.

% TODO: clean these up
\usetikzlibrary[calc]
% \usetikzlibrary[decorations.pathreplacing]
% \usetikzlibrary{decorations.pathmorphing}
% \usetikzlibrary[decorations.markings]
% \usetikzlibrary[arrows.meta]

\pgfqkeys{/kD}{
%==[ universal styles ]=========================================================
  every diagram/.append style={},
  every layout/.append style={square},
  every object/.append style={},
  every arrow/.append style={
    >=stealth,
  },
  every label/.append style={
    auto,
    inner sep=0.5ex,
    font=\everymath\expandafter{\the\everymath\scriptstyle}
  },
%==[ arrow styles ]=============================================================
  /kD/arrows/.cd,
    crossing over/clearance/.initial=0.5ex,
    crossing over/color/.initial=white,
    crossing over/.style={
      /tikz/preaction={
        -,
        draw=\pgfkeysvalueof{/kD/arrows/crossing over/color},
        line width=\pgfkeysvalueof{/kD/arrows/crossing over/clearance},
      },
    },
    shove/.style={
      /tikz/transform canvas={
        /tikz/shift={($(\tikztostart)!#1!-90:(\tikztotarget)-(\tikztostart)$)}
      }
    },
    slide/.style={
      /tikz/transform canvas={
        /tikz/shift={($(\tikztostart)!#1!0:(\tikztotarget)-(\tikztostart)$)}
      }
    },
%==[ label styles ]=============================================================
  /kD/labels/.cd,
    mid/.style={
      /tikz/fill=white,
      /tikz/shape=circle,
      /tikz/anchor=center,
      /tikz/inner sep=.25ex
    },
%=[ objects styles ]============================================================
  /kD/objects/.cd,
    % TODO: reflect on these styles
    % rectangular/.style 2 args={
    %   /tikz/node distance=#2 and #1
    % },
    % square/.style={
    %   /kD/objects/rectangular={#1}{#1}
    % },
    % golden/.style={
    %   /kD/objects/rectangular={#1}{0.618*#1}
    % },
    % % comb/.style={
    % %   /kD/objects/rectangular={#1}{sqrt(3/4)*#1},
    % % },
    % % comb/.default=4em,
    % square/.default=4em,
    % golden/.default=4em,
%=[ lattice styles ]============================================================
  /kD/layouts/.cd,
    rectangular/.style 2 args={
      /tikz/column sep={#1,between origins},
      /tikz/row sep={#2,between origins},
    },
    square/.style={
      /kD/layouts/rectangular={#1}{#1}
    },
    golden/.style={
      /kD/layouts/rectangular={#1}{0.618*#1}
    },
    comb/.code args={#1step #2 angle #3}{
      % TODO: write better option parser
      \if\relax#1\pgfkeys{/kD/layouts/horizontal comb=step #2 angle #3}
      \else\pgfkeys{/kD/layouts/#1comb=step #2 angle #3}\fi
    },
    horizontal comb/.style args={step #1 angle #2}{
      /kD/layouts/rectangular={#1}{tan(#2)*#1*0.5},
      /tikz/every odd row/.append style={/tikz/xshift=(#1)*0.5}
    },
    vertical comb/.style args={step #1 angle #2}{
      /kD/layouts/rectangular={tan(#2)*#1*0.5}{#1},
      /tikz/every odd column/.append style={/tikz/yshift=-1*(#1)*0.5}
    },
    comb/.default=step 4.5em angle 60,
    horizontal comb/.default=step 4.5em angle 60,
    vertical comb/.default=step 4.5em angle 60,
    square/.default=4.5em,
    golden/.default=4.5em,
%=[ diagram styles ]============================================================
  /kD/diagrams/.cd,
    grid/.style 2 args={
      /tikz/x={#1},
      /tikz/y={#2},
      /tikz/on grid
    },
    metric/.style 2 args={
      % {1 and 1}{1} is infty-norm, unit circle is unit square
      % {2}{0.5} is 1-norm, circle of radius 2 is rhombus circumscribing base hexagon
      /tikz/node distance={#1},
      % TODO: implement control to allow for explicit units on single factor specs
      /tikz/above left/.code={\tikz@lib@place@handle@{##1}{south east}{-1}{1}{north west}{#2}},
      /tikz/above right/.code={\tikz@lib@place@handle@{##1}{south west}{1}{1}{north east}{#2}},
      /tikz/below left/.code={\tikz@lib@place@handle@{##1}{north east}{-1}{-1}{south west}{#2}},
      /tikz/below right/.code={\tikz@lib@place@handle@{##1}{north west}{1}{-1}{south east}{#2}}
    },
    rectangular/.style 2 args={
      /kD/every layout/.append style={/kD/layouts/rectangular={#1}{#2}},
      % TODO: how much of the following is necessary in layouts?
      /kD/diagrams/grid={#1}{#2},
      /kD/diagrams/metric={1 and 1}{1}
    },
    square/.style={
      /kD/every layout/.append style={/kD/layouts/square={#1}},
      /kD/diagrams/grid={#1}{#1},
      /kD/diagrams/metric={1 and 1}{1}
    },
    golden/.style={
      /kD/every layout/.append style={/kD/layouts/golden={#1}},
      /kD/diagrams/grid={#1}{0.618*#1},
      /kD/diagrams/metric={1 and 1}{1}
    },
    comb/.code args={#1step #2 angle #3}{
      % TODO: write better option parser
      \if\relax#1\pgfkeys{/kD/diagrams/horizontal comb=step #2 angle #3}
      \else\pgfkeys{/kD/diagrams/#1comb=step #2 angle #3}\fi
    },
    horizontal comb/.style args={step #1 angle #2}{
      /kD/every layout/.append style={/kD/layouts/horizontal comb=step #1 angle #2},
      /kD/diagrams/grid={#1*0.5}{#1*tan(#2)*0.5},
      /kD/diagrams/metric={2}{0.5}
    },
    vertical comb/.style args={step #1 angle #2}{
      /kD/every layout/.append style={/kD/layouts/vertical comb=step #1 angle #2},
      /kD/diagrams/grid={#1*tan(#2)*0.5}{#1*0.5},
      /kD/diagrams/metric={2}{0.5}
    },
    comb/.default=step 4.5em angle 60,
    rectangular/.default={6em}{4em},
    square/.default=4.5em,
    golden/.default=4.5em,
}



==> tikzlibrarykodi.mitra.code.tex <==
%% tikzlibrarykodi.mitra.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% μήτρα • (mítra)
%   1. womb
%   2. matrix
%   3. mold

% Mitra is an alternative parsing mechanism for TiKz matrices of nodes.
% It couples with ozos to ensure the node contents  always pass through the TikZ key.

\usetikzlibrary{matrix}
\usetikzlibrary{kodi.koinos}

%==[ TikZ/pgf layer ]===========================================================

\pgfkeys{
  /mitra/every matrix/.style={
    /tikz/matrix,
    /tikz/cells={
      /tikz/anchor=base
    }
  },
  /mitra/every node/.style={},
  % NOTE: the alisa key *cannot* be put along with global node styles
  %   because order of execution.
  /mitra/matrix coordinates alias/.style={
    /tikz/alias=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn,
  }
}

%==[ main macro ]===============================================================

\def\kDMitra
  {\kDMitraFetchMatrixThen
  {\kDMitraParseMatrixTableThen
   \kDMitraOutput}}

% General purpose scratch register.
\newtoks\kDMitraTmpTok

%==[ fetching routine ]=========================================================

% I use the general one implemented by koinos.
\let\kDMitraFetchMatrixThen\kDFetchOptAndGrpThen

%==[ parsing routine: /table ]==================================================

\newtoks\kDMitraMatOutTok

\def\kDMitraParseMatrixTableThen#1{%
  \kDMitraMatOutTok={}%
  \expandafter\kDMitraParseTable\the\kDGrpTok\kD
  #1}

\def\kDMitraParseTable
  {\kDMitraParseAllRowsThen\relax}

\def\kDMitraParseAllRowsThen#1{%
  \def\kDExit{#1}%
  \kDIfNextHardCh\kD
    {\expandafter\kDExit\kDGobbleHardTok}%
    {\kDMitraParseOneRowThen{\kDMitraParseAllRowsThen{#1}}}}

%==[ parsing routine: /table/row ]==============================================

\def\kDMitraParseOneRowThen#1%
  {\kDMitraMarkRowEndBefore
  {\kDMitraParseAllColsThen
  {\kDMitraParseRowEndThen
  {#1}}}}

\begingroup\catcode`&=4 % ConTeXt hack
\gdef\kDMitraMarkRowEndBefore#1#2\\{#1#2&\kD\\}
\endgroup

\def\kDMitraParseAllColsThen#1{%
  \def\kDExit{#1}%
  \kDIfNextHardCh\kD
    {\expandafter\kDExit\kDGobbleHardTok}%
    {\kDMitraParseOneColThen{\kDMitraParseAllColsThen{#1}}}}

\def\kDMitraParseRowEndThen#1%
  {\kDMitraFetchRowEndThen
  {\kDMitraPrintRowEndThen
  {#1}}}

\def\kDMitraFetchRowEndThen#1\\{\kDMitraMaybeFetchRowOptionsThen{#1}}

\newtoks\kDMitraRowOptTok

\def\kDMitraPrintRowEndThen#1{%
  \edef\kDAct{\noexpand\kDMitraTmpTok={\noexpand\\\the\kDMitraRowOptTok}}%
  \kDAct
  \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
  #1}

\def\kDMitraMaybeFetchRowOptionsThen#1{%
  \kDMitraRowOptTok={}%
  \kDIfNextHardCh[%
    {\kDMitraFetchRowOptionsThen{#1}}%
    {#1}}

\def\kDMitraFetchRowOptionsThen#1[#2]{\kDMitraRowOptTok={[#2]}#1}

%==[ parsing routine: /table/row/column ]=======================================

\def\kDMitraParseOneColThen#1%
  {\kDMitraParseCellThen
  {\kDMitraParseColEndThen
  {#1}}}

\def\kDMitraParseColEndThen#1%
  {\kDMitraMaybeFetchColOptionsThen
  {\kDMitraMaybePrintColEndThen
  {#1}}}

\newtoks\kDMitraColOptTok

\def\kDMitraMaybeFetchColOptionsThen#1{%
  \kDMitraColOptTok={}%
  \kDIfNextHardCh[%
    {\kDMitraFetchColOptionsThen{#1}}%
    {#1}}

\def\kDMitraFetchColOptionsThen#1[#2]{\kDMitraColOptTok={[#2]}#1}

% TODO: make catcode change temporary with wrapping group and global defs
%   making sure auxiliary macros aren't botched (and don't botch anything).
\catcode`&=\active
\def\kDMitraMaybePrintColEndThen#1{%
  \kDIfNextHardCh\kD
    {#1}%
    {%
      \edef\kDAct{\noexpand\kDMitraTmpTok={\noexpand&\the\kDMitraColOptTok}}%
      \kDAct
      \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
      #1%
    }}
\catcode`&=4

%==[ parsing routine: /table/row/column/cell ]==================================

\def\kDMitraParseCellThen#1%
  {\kDMitraMaybeFetchCellOptionsThen
  {\kDMitraFetchCellContentThen
  {\kDMitraPrintCellThen
  {#1}}}}

\newtoks\kDMitraCelOptTok

\def\kDMitraMaybeFetchCellOptionsThen#1{%
  \kDMitraCelOptTok={}%
  \kDIfNextHardCh|%
    {\kDMitraFetchCellOptionsThen{#1}}
    {#1}}

\def\kDMitraFetchCellOptionsThen#1|#2|{\kDMitraCelOptTok={#2}#1}

\newtoks\kDMitraCelCntTok

\def\kDMitraFetchCellContentThen#1#2&{%
  \kDMitraCelCntTok={#2}%
  \kDTrimLeadingSpace\kDMitraCelCntTok
  \kDTrimTrailingSpace\kDMitraCelCntTok
  #1}

\def\kDMitraMaybeDoCellThen#1{%
  \kDIfNextHardCh\kD
    {#1}%
    {\kDMitraParseOneColThen{#1}}}

\def\kDMitraPrintCellThen#1{%
  \edef\kDAct{%
    \noexpand\kDMitraTmpTok={%
      \noexpand\node
        [/mitra/every node]%
        \the\kDMitraCelOptTok
        [node contents={\the\kDMitraCelCntTok},%
        /mitra/matrix coordinates alias];% NOTE: be careful about placement
      \kDMitraMaybeDumpCell}}%
  \kDAct
  \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
  #1}

%==[ dumping routine ]==========================================================

% TODO: revise the mechanism
\def\kDMitraMaybeDumpCell{\noexpand\pgfextra{%
  \noexpand\kDDump{'\noexpand\the\noexpand\pgfmatrixcurrentrow-\noexpand\the\noexpand\pgfmatrixcurrentcolumn':}%
  \noexpand\kDDump{\space\space options: '\the\kDMitraCelOptTok'}%
  \noexpand\kDDump{\space\space content: '\the\kDMitraCelCntTok'}}}

%==[ output routine ]===========================================================

\def\kDMitraOutput{%
  \edef\kDAct{%
    \noexpand\kDMitraTmpTok={%
      \noexpand\matrix
        [/mitra/every matrix]%
        \the\kDOptTok
        {\the\kDMitraMatOutTok};}}%
  \kDAct
  \the\kDMitraTmpTok}

%==[ notes ]====================================================================

% \newif\ifConTeXt
% Trick stolen from iftex. The second line is expanded inside the group so
% the global scope isn't polluted by \csname defining the token.
% \begingroup\expandafter\expandafter\expandafter\endgroup\expandafter
%   \ifx\csname starttext\endcsname\relax\ConTeXtfalse\else\ConTeXttrue\fi
% \ifConTeXt\catcode`|=12 \fi% TODO: why was the space necessary again?



==> tikzlibrarykodi.ozos.code.tex <==
%% tikzlibrarykodi.ozos.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% όζος • (ózos)
%   1. node
%   2. nodule
%   3. gnarl

% Ozos is an alternative parsing mechanism for TiKz nodes.
% It implements the following transformation
%   \kDOzos ... {CONTENTS};  --->  \node ... [node contents={CONTENTS}];
% to ensure the node contents always pass through the TikZ key.

\usetikzlibrary{kodi.koinos}

%==[ TikZ/pgf layer ]===========================================================

\pgfkeys{/ozos/every node/.style={}}

%==[ main macro ]===============================================================

\def\kDOzos%
  {\kDOzosFetchThen
  {\kDOzosMaybeDumpThen
   \kDOzosOutput}}

%==[ fetching routine ]=========================================================

% I use the general one implemented by koinos.
\let\kDOzosFetchThen\kDFetchOptAndGrpThen

%==[ parsing routine ]==========================================================

% Trivially solved by fetching.

%==[ dumping routine ]==========================================================

% TODO: revise the mechanism
\def\kDOzosMaybeDumpThen#1{%
  \kDDump{options: '\the\kDOptTok'}%
  \kDDump{content: '\the\kDGrpTok'}%
  #1}

%==[ output routine ]===========================================================

\def\kDOzosOutput{
  \edef\kDAct{
    \noexpand\node
      [/ozos/every node]
      \the\kDOptTok
      [/tikz/node contents={\the\kDGrpTok}];
  }
  \kDAct
}



==> tikzlibrarykodi.ramma.code.tex <==
%% tikzlibrarykodi.ramma.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% ράμμα • (rámma)
%   1. suture
%   2. catgut
%   3. stitch

% Ramma ties together the lower level libraries to define
% the user level functionality. NOTE: strictly no aesthetics, see mandyas.

\usetikzlibrary[kodi.bapto]
\usetikzlibrary[kodi.ektropi]
\usetikzlibrary[kodi.katharizo]
\usetikzlibrary[kodi.koinos]
\usetikzlibrary[kodi.ozos]
\usetikzlibrary[kodi.mitra]
\usetikzlibrary[kodi.velos]

% And here is the core idea of koDi itself:

\pgfqkeys{/tikz}{% TODO: is this the best scope to put the key into?
  self naming/.style={
    /tikz/node contents/.forward to=/bapto/input,
    /bapto/trigger/.forward to=/katharizo/input,
    /katharizo/output/.forward to=/bapto/dispatcher
  }
}

% Some mischief with handlers and baseline math/labeling functionality.

\pgfqkeys{/kD}{
  .search also=/bapto,
  .search also=/katharizo,
  every thing/.style={
    /ektropi/restore,
    /ektropi/add=/kD,
    /ektropi/add=/bapto,
    /ektropi/add=/katharizo,
  },
  every diagram/.style={% NOTE: restore hopefully unnecessary
    /kD/every thing,
    /ektropi/add=/kD/diagrams,
  },
  every layout/.style={% NOTE: restore unnecessary
    /kD/every thing,
    /ektropi/add=/kD/layouts,
    nodes={/kD/every object}
  },
  every object/.style={% NOTE: needed when inside matrices
    /kD/every thing,
    /ektropi/add=/kD/objects,
    execute at begin node=$,%
    execute at end node=$,%
    self naming,
  },
  every arrow/.style={% NOTE: restore unnecessary
    /kD/every thing,
    /ektropi/add=/kD/arrows
  },
  every label/.style={% NOTE: restore needed because inside edge
    /kD/every thing,
    /ektropi/add=/kD/labels,
    execute at begin node=$,%
    execute at end node=$,%
    self naming
  }
}

% The user level keys are bound to the underlying parsers.

\pgfkeys{
  /mitra/every matrix/.append style=/kD/every layout,
  /ozos/every node/.append style=/kD/every object,
  /velos/every path/.append style={
    /tikz/every edge/.append style=/kD/every arrow,
    /tikz/every edge quotes/.append style=/kD/every label
  }
}

% I merge the macro syntax for objects and matrices. Convenient!

\newif\ifkDRammaObjIsMatrix

\def\kDRammaObjDecideWhetherIsMatrixThen#1{%
  \def\kDRammaObjDWIM{\kDRammaObjDWIMSightThen{\kDRammaObjDWIMGobThen{#1}}}%
  \expandafter\kDRammaObjDWIM\the\kDGrpTok\\\kD}

\def\kDRammaObjDWIMSightThen#1#2\\%
  {\kDIfNextHardCh\kD
    {\kDRammaObjIsMatrixfalse#1}%
    {\kDRammaObjIsMatrixtrue#1}}

\def\kDRammaObjDWIMGobThen#1#2\kD{#1}

\def\kDRammaObjOutput
  {\ifkDRammaObjIsMatrix
    \kDMitraParseMatrixTableThen\kDMitraOutput\else
    \kDOzosOutput\fi}

\def\kDRammaObj
  {\kDFetchOptAndGrpThen
  {\kDRammaObjDecideWhetherIsMatrixThen
   \kDRammaObjOutput}}

% Just an identity.
\let\kDRammaMor\kDVelos

% I envelope the koDi main macros in a simple key for maximal flexibility.

\tikzset{
  kodi/.code={%
    \catcode`\|=12% ConTeXt hack TODO: is it sufficient? investigate
    \let\obj\kDRammaObj
    \let\mor\kDRammaMor
  },
  kodi/.append style={/kD/every diagram}
}

% TODO: not convinced by the structure of what follows

%==[ main macro ]===============================================================

\def\kDRamma
  {\kDRammaMaybeFetchOptionsThen
   \kDRammaOutput}

%==[ fetching routine ]=========================================================

\newtoks\kDRammaOptTok
\newtoks\kDRammaTmpTok

\def\kDRammaMaybeFetchOptionsThen#1{%
  \kDRammaOptTok={}%
  \kDIfNextHardCh[%
    {\kDRammaFetchOptionsThen{#1}}%
    {#1}}

\def\kDRammaFetchOptionsThen#1[#2]{\kDRammaOptTok={#2}#1}

%==[ output routine ]===========================================================

\def\kDRammaOutput{%
  \edef\kDAct{%
    \noexpand\kDRammaTmpTok={%
      \noexpand\tikzpicture[kodi, \the\kDRammaOptTok]}}%
  \kDAct
  \the\kDRammaTmpTok}

\let\kDRammaOpen\kDRamma
\let\kDRammaShut\endtikzpicture



==> tikzlibrarykodi.velos.code.tex <==
%% tikzlibrarykodi.velos.code.tex
%% Copyright 2017 Paolo Brasolin
%
% This file is part of 'koDi', hereafter referred as 'this work'.
% This file belongs to version v0.0.0 of this work.
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   <http://www.latex-project.org/lppl.txt>
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Paolo Brasolin
% who can be contacted at <paolo.brasolin@gmail.com>.
%
% This work consists of the following files, typically distributed in either
% a flat directory structure or the tree directory structure described below:
%
%   tex/plain/kodi/
%    ╰╴kodi.tex
%   tex/latex/kodi/
%    ╰╴kodi.sty
%   tex/context/third/kodi/
%    ╰╴t-kodi.tex
%   tex/generic/kodi/
%    ├╴tikzlibrarykodi.katharizo.code.tex
%    ├╴tikzlibrarykodi.code.tex
%    ├╴tikzlibrarykodi.ramma.code.tex
%    ├╴tikzlibrarykodi.ektropi.code.tex
%    ├╴tikzlibrarykodi.ozos.code.tex
%    ├╴tikzlibrarykodi.koinos.code.tex
%    ├╴tikzlibrarykodi.mandyas.code.tex
%    ├╴tikzlibrarykodi.bapto.code.tex
%    ├╴tikzlibrarykodi.diorthono.code.tex
%    ├╴tikzlibrarykodi.mitra.code.tex
%    ╰╴tikzlibrarykodi.velos.code.tex
%   doc/generic/kodi/
%    ├╴kodi-doc.tex
%    ├╴kodi-doc.pdf
%    ╰╴README
%
% Further informations about this work can be found at the following links:
%
%   https://ctan.org/pkg/kodi
%    ╰╴download, read generalities
%   http://mirror.ctan.org/graphics/pgf/contrib/kodi
%    ╰╴download, browse the files
%   https://paolobrasolin.github.io/kodi
%    ╰╴homepage
%   https://github.com/paolobrasolin/kodi
%    ╰╴Github repository
%

% βέλος • (vélos)
%   1. arrow
%   2. dart
%   3. shaft

% Velos is a parsing mechanism for arrow chains.

\usetikzlibrary{kodi.koinos}

%==[ handlers ]=================================================================

\pgfkeys{
  /velos/install quote handler/.style={
    /handlers/first char syntax=true,
    % TODO: verify if I can actually work w/quotes instead of against it
    /handlers/first char syntax/the character "/.initial=\kDVelosQuoteHandler
    % node quotes mean={node contents={#1}},
    % edge quotes mean={node contents={#1}}
  }
}

\def\kDVelosQuoteHandler#1%
  {\pgfkeysalso{/tikz/node contents/.expand once={\kDVelosUnquote#1}}}

\def\kDVelosUnquote"#1"{#1}

%==[ global options ]===========================================================

\newtoks\kDVelosTemp

\newtoks\kDVelosGlobalLabelOptions
\newtoks\kDVelosGlobalEdgeOptions

\newif\ifkDVelosGOAfterColon

\def\kDVelosFetchGlobalOptionsThen#1{%
  \kDVelosGOAfterColonfalse
  \kDVelosGlobalLabelOptions={}%
  \kDVelosGlobalEdgeOptions={}%
  \kDVelosGOMaybeFetchThen{\kDVelosGOThinkThen{#1}}}

\def\kDVelosGOMaybeFetchThen#1{%
  \kDVelosTemp={}%
  \kDIfNextHardCh[%
    {\kDVelosGOFetchThen{#1}}%
    {#1}}

\def\kDVelosGOFetchThen#1[#2]{%
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosGOThinkThen#1{%
  \def\kDVelosGOLoop{\kDVelosGOThinkThen{#1}}%
  \def\kDVelosGOBreak{#1}%
  \kDIfNextHardCh:%
    {%
      \kDVelosGOAfterColontrue
      \kDVelosGlobalLabelOptions\expandafter{\the\kDVelosTemp}%
      \expandafter\kDVelosGOMaybeFetchThen\expandafter\kDVelosGOLoop\kDGobbleHardTok
    }{%
      \ifkDVelosGOAfterColon
        \kDVelosGlobalEdgeOptions\expandafter{\the\kDVelosTemp}\else
        \kDVelosGlobalLabelOptions\expandafter{\the\kDVelosTemp}\fi
      \kDVelosGOBreak
    }}

%==[ first edge ]===============================================================

\def\kDVelosDoFirstEdgeThen#1%
  {\kDVelosFetchFirstSourceThen
  {\kDVelosFetchFirstEdgeThen
  {\kDVelosDrawFetchedEdgeThen
  {#1}}}}

\newtoks\kDVelosSource
\newtoks\kDVelosCurFstSrc
\newtoks\kDVelosPrvFstSrc

\def\kDVelosFetchFirstSourceThen#1%
  {\kDIfNextHardCh(%
    {\kDVelosFFSBracketsThen{#1}}%
    {\kDVelosFFSTillOverThen{#1}}}

\def\kDVelosFFSBracketsThen#1(#2){%
  \kDVelosSource={#2}%
  \kDVelosCurFstSrc={#2}%
  #1}

\def\kDVelosFFSTillOverThen#1#2 {% <- mind the space!
  \kDVelosSource={#2}%
  \kDVelosCurFstSrc={#2}%
  #1}

\def\kDVelosFetchFirstEdgeThen#1%
  {\kDVelosFetchEdgeThen
  {\kDVelosFetchTargetThen
  {#1}}}

%==[ chained edges ]============================================================

\newtoks\kDVelosEdge

\def\kDVelosFetchEdgeThen#1{%
  \kDVelosEdge={}%
  \kDVelosFEThen{\kDVelosFEThinkThen{#1}}}

\def\kDVelosFEThen#1%
  {\kDIfNextHardCh[%
    {\kDVelosFEKeysListThen{#1}}%
    {\kDIfNextHardCh"%
      {\kDVelosFEEnquotedThen{#1}}%
      {\kDVelosFETillOverThen{#1}}}}

\newif\ifkDVelosTempIsKeysList

\def\kDVelosFEEnquotedThen#1"#2"{%
  \kDVelosTempIsKeysListfalse
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosFEKeysListThen#1[#2]{%
  \kDVelosTempIsKeysListtrue
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosFETillOverThen#1{%
  \kDVelosTempIsKeysListfalse
  \kDVelosTemp={}%
  \kDVelosFETOThen{#1}}

\def\kDVelosFETOThen#1%
  {\kDIfNextSoftCh\kDBlankSpace
    {#1}%
    {\kDIfNextHardCh:%
      {#1}
      {\kDVelosFEAppendThen{\kDVelosFETOThen{#1}}}}}

\def\kDVelosFEAppendThen#1#2{%
  \kDVelosTemp=\expandafter{\the\kDVelosTemp#2}% TODO: wasn't the \ea redundant?
  #1}

\def\kDVelosFEEdgePrepend#1{%
  \edef\Act{\noexpand\kDVelosEdge={#1,\the\kDVelosEdge}}%
  \Act}

\def\kDVelosFEEdgePrependNode#1%
  {\kDVelosFEEdgePrepend{edge node={node[every edge quotes][/velos/install quote handler,#1]}}}
% TODO: install quote handler is maximally local to avoid conflict with quotes library;
%   is this the best handling of the situation?

\def\kDVelosFEThinkThen#1{%
  \def\kDVelosFELoop{\kDVelosFEThinkThen{#1}}%
  \def\kDVelosFEBreak{#1}%
  \kDIfNextHardCh[%
    {%
      \kDVelosFEEdgePrependNode{\the\kDVelosTemp}%
      \kDVelosFEThen\kDVelosFELoop
    }{%
      \kDIfNextHardCh:%
        {%
          \ifkDVelosTempIsKeysList
            \kDVelosFEEdgePrependNode{\the\kDVelosTemp}\else
            \kDVelosFEEdgePrependNode{"\the\kDVelosTemp"}\fi
          \expandafter\kDVelosFEThen\expandafter\kDVelosFELoop\kDGobbleHardTok
        }{%
          \kDVelosFEEdgePrepend{\the\kDVelosTemp}%
          \kDVelosFEBreak
        }%
    }}

%==[ target ]===================================================================

\newtoks\kDVelosTarget
\newtoks\kDVelosCurLstTar
\newtoks\kDVelosPrvLstTar

\def\kDVelosFetchTargetThen#1%
  {\kDIfNextHardCh(%
    {\kDVelosFTBracketsThen{#1}}%
    {\kDVelosFTTillOverThen{#1}}}

\def\kDVelosFTBracketsThen#1(#2){%
  \kDVelosTarget={#2}%
  \kDVelosCurLstTar={#2}%
  #1}

\def\kDVelosFTTillOverThen#1{%
  \kDVelosTarget={}%
  \kDVelosFTTOThen{#1}}

\def\kDVelosFTTOThen#1{%
  \def\kDVelosFTTOLoop%
    {\kDVelosFTTOThen{#1}}%
  \def\kDVelosFTTOExit{%
    \kDVelosCurLstTar\expandafter{\the\kDVelosTarget}%
    #1}%
  \kDIfNextSoftCh\kDBlankSpace
    {\kDVelosFTTOExit}%
    {\kDIfNextHardCh;%
      {\kDVelosFTTOExit}%
      {\kDVelosFTAppendThen\kDVelosFTTOLoop}}}

\def\kDVelosFTAppendThen#1#2{%
  \kDVelosTarget=\expandafter{\the\kDVelosTarget#2}%
  #1}

%==[ rendering/dereferencing ]==================================================

\def\kDVelosAlias{*}
\def\kDVelosSaila{+}

\newtoks\kDVelosDerefSrc
\newtoks\kDVelosDerefTar

\def\kDVelosDrawFetchedEdgeThen#1{
  \edef\cS{\the\kDVelosSource}%
  \kDVelosDerefSrc\expandafter{\the\kDVelosSource}%
  \ifx\cS\kDVelosAlias\kDVelosDerefSrc\expandafter{\the\kDVelosPrvFstSrc}\fi
  \ifx\cS\kDVelosSaila\kDVelosDerefSrc\expandafter{\the\kDVelosPrvLstTar}\fi
  \edef\cT{\the\kDVelosTarget}%
  \kDVelosDerefTar\expandafter{\the\kDVelosTarget}%
  \ifx\cT\kDVelosAlias\kDVelosDerefTar\expandafter{\the\kDVelosPrvLstTar}\fi
  \ifx\cT\kDVelosSaila\kDVelosDerefTar\expandafter{\the\kDVelosPrvFstSrc}\fi
  \edef\Act{%
    \noexpand\path
      [/velos/every path]%
      [%
        /tikz/every edge/.append style=%
          {\the\kDVelosGlobalEdgeOptions},%
        /tikz/every edge quotes/.append style=%
          {auto,\the\kDVelosGlobalLabelOptions},%
      ]%
      (\the\kDVelosDerefSrc)%
      edge[\the\kDVelosEdge]%
      (\the\kDVelosDerefTar);}%
  \Act%
  #1}

\pgfkeys{
  /velos/every path/.style={
    /velos/install quote handler
  }
}

%==[ high level ]===============================================================

\def\kDVelos%
  {\kDVelosFetchGlobalOptionsThen
  {\kDVelosDoFirstEdgeThen
   \kDVelosMaybeChainEdge}}

\def\kDVelosMaybeChainEdge{%
  \kDIfNextHardCh;%
    {%
    \edef\cS{\the\kDVelosCurFstSrc}%
    \ifx\cS\kDVelosAlias
      \kDVelosCurFstSrc\expandafter{\the\kDVelosPrvFstSrc}%
    \else\ifx\cS\kDVelosSaila
      \kDVelosCurFstSrc\expandafter{\the\kDVelosPrvLstTar}%
    \fi\fi
    \edef\cT{\the\kDVelosCurLstTar}%
    \ifx\cT\kDVelosAlias
      \kDVelosCurLstTar\expandafter{\the\kDVelosPrvLstTar}%
    \else\ifx\cT\kDVelosSaila
      \kDVelosCurLstTar\expandafter{\the\kDVelosPrvFstSrc}%
    \fi\fi
    \kDVelosPrvFstSrc\expandafter{\the\kDVelosCurFstSrc}%
    \kDVelosPrvLstTar\expandafter{\the\kDVelosCurLstTar}%
    }{%
      \kDVelosSource\expandafter{\the\kDVelosTarget}
      \kDVelosFetchEdgeThen
        {\kDVelosFetchTargetThen
        {\kDVelosDrawFetchedEdgeThen
         \kDVelosMaybeChainEdge}}%
    }}


